Approximating the Expected Values for Combinatorial Optimization Problems over Stochastic Points

We consider the stochastic geometry model where the location of each node is a random point in a given metric space, or the existence of each node is uncertain. We study the problems of computing the expected lengths of several combinatorial or geometric optimization problems over stochastic points, including closest pair, minimum spanning tree, $k$-clustering, minimum perfect matching, and minimum cycle cover. We also consider the problem of estimating the probability that the length of closest pair, or the diameter, is at most, or at least, a given threshold. Most of the above problems are known to be $\sharpP$-hard. We obtain FPRAS (Fully Polynomial Randomized Approximation Scheme) for most of them in both the existential and locational uncertainty models. Our result for stochastic minimum spanning trees in the locational uncertain model improves upon the previously known constant factor approximation algorithm. Our results for other problems are the first known to the best of our knowledge.

==> app-convexhull.tex <==
\section{Convex Hull (2D)}
\label{app:ch}

We demonstrate the problem of computing the expected area of the convex hull (2D) under the {\em existential uncertainty model}. Given a set of points $\P=\{s_1, \ldots, s_m\}$ on a plane, where each point $s_i\in \P$ is present with probability $p_i$. For any nonnegative integer $i$ and a point set $H$, let $H\A{i}$ to denote the event that exactly $i$ points are present in $H$.

We use $\CH$ to denote the the expected area of the convex hull in the realized graph. Our \core\ recipe works well for this problem.
Firstly, we find the \core\ $\H=\{s_i\mid p_i\geq \frac{\e}{m^2}\}$. Let $\calF=\P\setminus \H$. Then we could rewrite $\Exp[\CH]$ by $\sum_{0\leq i\leq m}\Prob[\calF\A{i}]\cdot \Exp[\CH\mid \calF\A{i}]$. We need the following lemma first.

\begin{lemma}
\label{lm:4ch}
Given a convex hull with no less than 4 points whose aero is $A$. There exists 4 points on the convex hull, where the aero of the convex hull constructed by these 4 points is at least $A/2$.
\end{lemma}

\begin{proof}
We find the farthest pair ($s_1,s_2$) on the convex hull at first. Connect $s_1$ and $s_2$ to get a straight line $l$. On both sides of $l$, find a point each on the convex hull which is the farthest from $l$. Suppose these 2 points are $s_3$ and $s_4$, then by the property of convex hull, the aero of the convex hull constructed by $s_1,s_2,s_3,s_4$ is at least $A/2$.
\qed
\end{proof}

By Lemma~\ref{lm:4ch}, we could use the similar argument as $\Prob[\CP\leq 1]$ to show the contribution of the term $\sum_{5\leq i\leq n}\Prob[\calF\A{i}]\cdot \Exp[\CH\mid \calF\A{i}]$ are negligible compared to the fifth term. Briefly speaking, for $i\geq 5$ and a realized graph $C$ conditioning on $\calF\A{i}$, we could find out a realized graph conditioning on $\calF\A{i-1}$ which is of aero at least $\CH(C)/2$.
Then we just use the Monte Carlo method to estimate the first five terms and achieve an $\FA$ for the problem.


==> app-matching.tex <==
\section{Missing Details for Section~\ref{sec:mm}: Minimum Perfect Matching}
\label{app:matching}






\topic{Finding \core}
We need the following lemma which is useful in bounding $\Exp[\MM]$ from below.
\begin{lemma}
\label{lm:lm2core}
For any two disjoint sets $H_1$ and $H_2$ of points, and any node $v$,
we have
$$\Exp[\MM]\geq \min\{p_v(\H_1),p_v(\H_2)\}\cdot \dist(\H_1,\H_2)/m.$$
\end{lemma}


\begin{proof}
Suppose $s =\arg\max_{s'} \{p_{vs'}\mid s' \in \H_1\}$,
and $t =\arg\max_{t'}\{p_{vt'}\mid t' \in \H_2\}$.
Obviously, we have $p_{vs} \geq \frac{p_v(\H_1)}{m}$ and $p_{vt} \geq \frac{p_v(\H_2)}{m}$.
So it suffices to show $\Exp[\MM]\geq \min\{p_{vs},p_{vt}\}\cdot \dist(s,t)$.
We first see that
\begin{align*}
\Exp[\MM]&\geq p_{vs} \Exp[\MM\mid v \realize s]+ p_{vt} \Exp[\MM\mid v \realize t] \\
&\geq \min\{p_{vs},p_{vt}\} \Bigl(\Exp[\MM\mid v \realize s]
+\Exp[\MM\mid v \realize t]\Bigr).
\end{align*}
Then it is sufficient to prove that $\Exp[\MM\mid v \realize s]+\Exp[\MM\mid v \realize t]\geq \dist(s,t)$.
Fix a realization of all nodes except $v$ and condition on this event.
Consider the two minimum perfect matchings, one for the case $v \realize s$, (denoted as $\MM_1$) and
the other one for $v \realize t$ (denoted as $\MM_2$).
Consider the symmetric difference
$$\MM_1\oplus \MM_2:=(\MM_1\setminus \MM_2)\cup (\MM_2\setminus \MM_1).$$
We can see that it is a path $(s, p_1, p_2, \ldots,p_k ,t)$, such that $(s,p_1)\in \MM_1$,$(p_1,p_2)\in \MM_2,\ldots,$ $(p_k,t)\in \MM_2$.
So $\MM_1+\MM_2 \geq  \dist(s,t)$ by the triangle inequality.
Therefore, we have $\Exp[\MM\mid v \realize s]+\Exp[\MM\mid v \realize t]\geq \dist(s,t)$.
\qed
\end{proof}

By Q1, Q2 and the above lemma, we can show the following additional property holds.

\vspace{0.2cm}
\noindent
{\bf Lemma~\ref{lm:estMMhome}\,\,\,}
{\em
Q3. \,\,$\Exp[\MM]=\Omega(\frac{\e D}{nm^5})$
where $D=\max_i\{\diam(\H_i)\}$.
}
\vspace{0.1cm}

\begin{proof}
Note that the stopping point $T$ must exist, because the set of all points satisfies the first two properties.
Now, we show the Q3 also holds.
Recall $D=\max_i \diam(\H_i)$.
Firstly, note that $D\leq 2mT$.
Secondly, consider $T'=T-\varepsilon$ for some infinitesimal $\varepsilon>0$.
At time $T'$, consider two situations:
\begin{enumerate}
\item There exists a node $v$, such that
$\forall j, p_v(\H_j)< 1-O(\frac{\e}{nm^3})$.
Then there must exist two components $C_1$ and $C_2$ such that $p_v(C_1) > \Omega(\frac{\e}{nm^3})$
and $p_v(C_2) > \Omega(\frac{\e}{nm^3})$.
Moreover, since $C_1$ and $C_2$ are two distinct components, $\dist(C_1,C_2)\geq 2T'$.
Then, by Lemma~\ref{lm:lm2core}, we have $\Exp[\MM]\geq \Omega(\frac{\e}{nm^4}) \cdot 2T\geq \Omega(\frac{\e}{nm^5})$.
\item Suppose the Q1 is true but Q2 is still false.
Suppose $\H_j$ is a component which homes odd number of nodes.
We note that with probability at least $(1-\frac{1}{nm^3})^{n}\approx 1$,
every node realizes to a point in its home.
When this is the case, there is at least one node in $\H_j$ that needs to be matched
with some node outside $\H_j$, which incurs a cost of at least
$2T$. \qed
\end{enumerate}
\end{proof}

\topic{Estimating $\Exp[\MM]$}
Again, we only need to describe how to estimate the first two terms.
Our final estimation is simple the sum of the first two terms.

\linesnotnumbered
\begin{algorithm}[h]
\label{alg:estMM}
\caption{Estimating $\Exp[\,\MM\mid \calF\A{0} \,] \cdot \Prob[ \calF\A{0}]$}
\textbf{Estimating $\Exp[\,\MM\mid \calF\A{0} \,] \cdot \Prob[ \calF\A{0}]$}\\
\nl Take $N_1=O(\frac{n^2m^5}{\e^4}\ln n)$ independent samples. Set $A\leftarrow \emptyset$ at the beginning.\\
\nl For each sample $G_i$, if it satisfies $\H\A{n}$, $A\leftarrow A\cup \{G_i\}$.\\
$T_0\leftarrow \frac{1}{N_1}\sum_{G_i\in A}\MM(G_i)$.\\
\end{algorithm}
%\vspace{-0.6cm}

\begin{lemma}\label{lm:est0MM}
Algorithm~\ref{alg:estMM} produces a $(1\pm\epsilon)$-estimate for the first term with high probability.
\end{lemma}

\begin{proof}
Note that $\Prob[\H\A{n}]$ is close to $1$ (by union bound) and can be computed exactly.
To estimate $\Exp[\MM\mid \H\A{n}]]$, the algorithm takes the average of $N_1=O(\frac{n^2m^5}{\e^4}\ln n)$ samples. Note that conditioned on $\H\A{n}$, the minimum perfect matching could be at most $nD$.
We distinguish the following two cases.
\begin{enumerate}
\item
$\Exp[\MM\mid \H\A{n}]\geq \frac{\e}{2}\Exp[\MM]\geq\Omega(\frac{\e^2 D}{nm^5})$. We could get a $(1\pm \epsilon)$-approximation using the Monte Carlo method with $O(\frac{n^2m^5}{\e^4}\ln n)$ samples. This is because the maximum possible $\MM$ length is at most $nD$ and therefore we have poly-bounded.
\item
$\Exp[\MM\mid \H\A{n}]< \frac{\e }{2}\Exp[\MM]$. Then the probability that the sample average is larger than $\epsilon \Exp[\MM]$ is at most $\poly(\frac{1}{n})$ by Chernoff Bound.
We can thus ignore this part safely. \qed
\end{enumerate}
\end{proof}

\vspace{-0.3cm}
\begin{algorithm}[h]
\label{alg:estMM2}
\caption{Estimating $\Exp[\,\MM\mid \calF\A{1} \,] \cdot \Prob[ \calF\A{1}]$}
\nl For each node $v$, set $B_v\leftarrow \{s\mid s\in \calF, \dist(s,\H(v))<\frac{4nD}{\e }$. Let $\Cl(v)$ be the event that $v$ is the only node that realizes to some node $s\notin \H(v)$ and $s\in B_v$.\\
\nl Conditioning on $\Cl(v)$, take $N_1=O\bigl( \frac{n^2m^5}{\e^{5}}\ln n\bigr)$ independent samples.
Let $A_v\leftarrow \{G_{v,i}\mid 1\leq i\leq N_2\}$ be the set of $N_1$ samples for $\Cl(v)$.\\
\nl $T_v\leftarrow \frac{1}{N_1}\sum_{G_{v,i}\in A_v}\MM(G_{v,i})$  ~~~(estimating $\Exp[\,\MM\mid \Cl(v)]$)\\
\nl $T_1\leftarrow \sum_{v\in \V}\Bigl(\Prob[\Cl(v)]T_v+\sum_{s\in \calF\setminus B_v}\Prob[\calF\A{v}\wedge v\realize s]\,\dist(s,\H(v))\,\Bigr)$.\\
\end{algorithm}
%\vspace{-0.3cm}


\begin{lemma}\label{lm:est1MM}
Algorithm~\ref{alg:estMM} produces a $(1\pm\epsilon)$-estimate for the second term with high probability.
\end{lemma}

\begin{proof}
To compute the second term, we first rewrite it as follows:
$$\Exp[\MM\mid \calF\A{1} ]\cdot \Prob[\H\A{1}]
=\sum_{v\in \V} \Bigl(\,\sum_{s\notin \Home(v)} \Prob[\calF\A{v}\wedge v\realize s]\
\Exp[\MM\mid \calF\A{v}, v\realize s ]\,\Bigr).
$$
%We can easily see that $\Prob[F\A{v}\wedge v\realize s]$ can be computed precisely in poly-time.
Fix a particular node $v$.
To estimate $\sum_{s\in \calF} \Prob[\calF\A{v}\wedge v\realize s]\, \Exp[\MM\mid \calF\A{v}, v\realize s ]$, we consider the following two situations:
\begin{enumerate}
\item
Point $s\in B^v$, i,e, $\dist(s,\H(v))<\frac{4nD}{\e }$.

We estimate the sum for all $s\in B^v$. Notice that the sum is
in fact $\Prob[\Cl(v)]\cdot\E[\,\MM\mid \Cl(v) ]$.
%Here $v\realize \Cl(s)$ means that node $v$ is present at some point $s\in \Cl(s)$.
We can see that $\Prob[\Cl(v)]$ can be computed exactly in linear time.
We argue the quality of the estimation taken on $N_2=O\bigl( \frac{n^2m^5}{\e^{5}}\ln n\bigr)$ samples is good
by considering the following two cases:
%If
%$$\sum_{s:\dist(u,H)<n^{10}}\Exp[\,\MST \mid F\A{v}, v\realize s ]\cdot\Prob[v\realize s \mid F\A{v}]
%\geq \frac{1}{n^3}\Exp[\,\MST \mid H\A{n}]]\geq \frac{1}{(mn)^5}\diam(H),
%$$
    \begin{enumerate}
    \item Assume that $
    \E[\,\MM\mid \Cl(v) ]
    \geq \frac{1}{2}\Exp[\,\MM \mid \H\A{n}]\geq \Omega\Bigl(\frac{\e D}{nm^5}\Bigr).
    $
    In this case, we have poly-bounded.
    This is because under the condition $\Cl(v)$,
    the maximum possible length of any minimum spanning tree is $O(\frac{nD}{\e})$.
    Hence we can use Monte Carlo to get a $(1\pm \epsilon)$-approximation
    of $\E[\,\MM\mid \Cl(v) ]$ with $O\bigl( \frac{nm^2}{\e^{5}}\ln n\bigr)$ samples.
    \item Otherwise, we assume that

    $
    \E[\,\MM\mid \Cl(v) ]
    \leq \frac{1}{2}\Exp[\,\MM \mid \H\A{n}]].
    $
    The probability that the sample average is larger than $\Exp[\MM\mid \H\A{n}]] $
    is at most $\poly(\frac{1}{n})$ by Chernoff Bound. The probability that for all nodes $v$, the sample average are
    at most $\Exp[\MM\mid \H\A{n}]]$ is at least $1-\poly(\frac{1}{n})$ by union bound.
    If this is the case, we can see their total contribution
    to the final estimation of $\E[\MM]$ is less than $\e \Exp[\,\MM \mid \H\A{n}]] \Prob[\H\A{n}] $.
    In fact, this is because
    \begin{align*}
    & \sum_{v\in V} \Prob[\Cl(v)]\cdot\E[\,\MM\mid \Cl(v) ]\leq \sum_{v\in V}\Prob[\Cl(v)]\cdot \Exp[\,\MM \mid \H\A{n}]] \\
    & <\e \Exp[\,\MM \mid \H\A{n}]] \Prob[\H\A{n}].
    \end{align*}
    The second inequality is due to the fact that $\sum_{v\in V}\Prob[\Cl(v)]\leq n-\sum_{v\in V} p_v(\H(v))\leq \frac{\e}{m^3}<\e \Prob[\H\A{n}]$.
    \end{enumerate}
\item
Point $s\in F\setminus B^v$, each term has $\dist(s,\H(v))>\frac{4nD}{\e }$.
The algorithm uses $\dist(s,\H(v))$
as the estimation of $\Exp[\MM\mid \calF\A{v}, v\realize s ]$.
Note that the length of $\MM$ is always at least $\dist(s,\H(v))-nD\geq (1-\frac{\e}{4})\dist(s,\H(v))$. This is because such an instance $\MM$ contains a path from $s$ to some point $t\in \H(v)$ deleting no more than $n$ segments of length at most $D$ (each segment is in some $\H_j$).
On the other hand, at most $\dist(s,\H(v))+nD \leq (1+\frac{\e}{4}) \dist(s,\H(v))$. So it is a $(1\pm\epsilon)$-estimation.
\qed
\end{enumerate}
\end{proof}

\topic{Analysis}
We show for $i>1$, the contribution from event $\calF\A{i}$ is negligible.
Suppose $S$ is the set of nodes that are out of their homes.
We use $\calF_S$ and $\calH_{\bS}$
to denote the set of all realizations of the all nodes in $S$ to points in $\calF$,
and the set of realizations of $\bS=V\setminus S$ to points in $\H$ respectively.
We use $\MM(F_S, H_{\bS})$ to denote the length of the minimum perfect matching
under the realization $(F_S, H_{\bS})$, where $F_S\in \calF_S$ and $H_{\bS}\in \calH_{\bS}$.
The following combinatorial fact plays the same role
in the charging argument as Lemma~\ref{lm:mstchange} does in the previous section.
Different from the MST problem,
we can not achieve a similar bound to the one in Lemma~\ref{lm:mstchange} since
$\MM(F_S, H_{\bS})$ may decrease significantly if we only sending only one node outside home back to its home.
However, we show that in such case, if we send one more node back home,
$\MM(F_S, H_{\bS})$ can still be bounded.

We need the following structural result about minimum perfect matchings,
which is essential for our charging argument.

\begin{lemma}
\label{lm:del1or2}
%A pair $(F_S,H_{\bS})$ means for each node $s\in S$,
%$s$ locates on a certain point out of $\textcircled{s}$, and for each node $s\in \bar{s}$, $s\realize \textcircled{s}$.
Fix a realization $(F_S,H_{\bS})$.
We use  $\ell(v)$ to denote $\dist(v, \Home(v))$ for all nodes $v\in S$.
Suppose $v_1\in S$ has the smallest $\ell$ value and $v_2$ has the second smallest $\ell$ value.
Let $S'=S\setminus \{v_1\}$, $S''=S'\setminus \{v_2\}$.
Further let $(F_{S'}, H_{\bS'})$ be a realization obtained from $(F_S, H_{\bS})$ by sending $v_1$ to
a point in its home $\Home(v_1)$
and
$(F_{S''}, H_{\bS''})$ be a realization obtained from $(F_{S'}, H_{\bS'})$ by sending $v_2$ to
a point in its home $\Home(v_2)$.
Then we have that
$
\MM(F_S,H_{\bS})\leq 2(m+2)\MM(F_{S'},H_{\bS'})+2(m+2)\MM(F_{S''},H_{\bS''})
$
\end{lemma}

\begin{proof}
Let $\d=\min_v \ell(v)$ and $D=\max_i \diam(H_i)$. Note that $d\geq \frac{D}{m}$ as $d\geq 2T$ and $D\leq 2mT$.
We distinguish the following three cases:
\begin{enumerate}
\item
$\MM(F_S,H_{\bS})\leq \frac{\d}{2}$.
Using a similar argument to the one in Lemma~\ref{lm:lm2core}, we have
$$
\MM(F_{S'},H_{\bS'})+\MM(F_S,H_{\bS})\geq \ell(v)=\d
$$
So, we have  $\MM(F_S,H_{\bS})\leq \MM(F_{S'},H_{\bS'})$ in this case.
\item
$\MM(F_S,H_{\bS})\geq (m+2)\d$.
%Let $s_1$ locate on a point in its corresponding ball. We can get a matching for $(F_{S^{'}},H_{\bar{S^{'}}})$.
By the triangle inequality,  we can see that
$$
\MM(F_{S'},H_{\bS'})+(m+1)d\geq \MM(F_{S'},H_{\bS'})+d+D\geq \MM(F_S,H_{\bS})
$$
So, we have $\MM(F_S,H_{\bS})\leq (m+2)\MM(F_{S'},H_{\bS'})$.
\item
$\frac{\d}{2}\leq \MM(F_S,H_{\bS})\leq (m+2)\d$.
\begin{enumerate}
\item
$\MM(F_{S'},H_{\bS'})\geq \frac{\d}{2}$.
We directly have $\MM(F_S,H_{\bS})\leq 2(m+2)\MM(F_{S'},H_{\bS'})$.
\item
$\MM(F_{S'},H_{\bS'})\leq \frac{\d}{2}$.
By Lemma~\ref{lm:lm2core}, we have
$$
\MM(F_{S'},H_{\bS'})+\MM(F_{S''},H_{\bS''})\geq \d
$$
Then we have $\MM(F_S,H_{\bS})\leq 2(m+2)\MM(F_{S''},H_{\bS''})$.
\end{enumerate}
\end{enumerate}
In summary, we prove the lemma. \qed
\end{proof}

What remains is to establish the following key lemma. The proof is
similar to, but more involved than that of Lemma~\ref{lm:mstcharge}.
\begin{lemma}
\label{lm:matchingcharge}
For any $\epsilon>0$,
if $\H$ satisfies the properties Q1, Q2 in Algorithm~\ref{alg:coreMM}, we have that
$$
\sum_{i> 1}\Exp[\MM\mid \calF\A{i}]\cdot \Prob[\calF\A{i}]\leq \epsilon\cdot \Exp[\MM\mid \calF\A{0}] \cdot \Prob[\calF\A{0}]+\epsilon\cdot \Exp[\MM\mid \calF\langle 1\rangle]\cdot \Prob[\calF\A{1}].
$$
\end{lemma}

\begin{proof}
We claim that for any $i > 1$,
$$
\Exp[\MM\mid \calF\A{i+1}]\cdot \Prob[\calF\A{i+1}]\leq
\frac{\epsilon}{6}\bigl(\,\Exp[\MM\mid \calF\A{i}]\cdot \Prob[\calF\A{i}]+\Exp[\MM\mid \calF\A{i-1}]\cdot \Prob[\calF\A{i-1}]\,\bigr)
$$
If the claim is true, the lemma can be proven easily as follows.
For ease of notation, we use $A(i)$ to denote $\Exp[\MM\mid \calF\A{i}]\cdot \Prob[\calF\A{i}]$.
First, we can see that
\begin{align*}
A(i+2)+A(i+1) \leq \frac{\epsilon}{6} A(i+1) +\frac{2\epsilon}{6}A(i) +\frac{\epsilon}{6} A(i-1)\leq \frac{\epsilon}{2}(A(i)+A(i-1)).
\end{align*}
So if $i$ is odd,
$A(i+2)+A(i+1) \leq (\frac{\epsilon}{2})^{(i+1)/2}(A(1)+A(0)).$
Therefore, $\sum_{i>1} A(i)\leq \frac{\epsilon/2}{1-\epsilon/2} (A(1)+A(0))\leq \e(A(1)+A(0))$.
%\begin{align*}
%& \leq \Bigl(\frac{3\epsilon}{n^2}\Bigr) \bigl(\,\Exp[\MM\mid F\A{i}]\cdot \Prob[F\A{i}]+\Exp[\MM\mid F\A{i-1}]\cdot \Prob[F\A{i-1}]\,\bigr)
%\end{align*}
%could use induction to prove an even stronger result.
%$$
%\sum_{i> 1}\Exp[\MM\mid F\A{i}]\cdot \Prob[F\A{i}]\leq (1-\frac{1}{n})\epsilon
%\cdot (\Exp[\MM\mid F\A{0}] \cdot \Prob[F\A{0}]+ \Exp[\MM\mid F\langle 1\rangle]\cdot \Prob[F\A{1}])
%$$
%The basic step: $n=2$, it's obvious. $n=3$, we have
%\begin{align*}
%&\Exp[\MM\mid F\A{3}]\cdot \Prob[F\A{3}]+\Exp[\MM\mid F\A{4}]\cdot \Prob[F\A{4}]\\
%\leq &(\frac{\epsilon}{4^2}+(\frac{\epsilon}{4^2})^2)\cdot(\Exp[\MM\mid F\A{0}] \cdot \Prob[F\A{0}]+(\frac{2\epsilon}{4^2}+(\frac{\epsilon}{4^2})^2)\cdot\Exp[\MM\mid F\langle 1\rangle]\cdot \Prob[F\A{1}]\\
%\leq &(1-\frac{1}{4})\epsilon \cdot (\Exp[\MM\mid F\A{0}] \cdot \Prob[F\A{0}]+ \Exp[\MM\mid F\langle 1\rangle]\cdot \Prob[F\A{1}])
%\end{align*}
%The induction step: If $n-1\geq 4$ is satisfied, then consider $n$ nodes.
%\begin{align*}
%\sum_{i=2}^{n}\Exp[\MM\mid F\A{i}]\cdot \Prob[F\A{i}]\leq
%& \Exp[\MM\mid F\A{0}]\cdot \Prob[F\A{0}]+ \sum_{i=1}^{n-2}\Exp[\MM\mid F\A{0}]\cdot \Prob[F\A{0}]
%\sum_{i=2}^{n-1}\Exp[\MM\mid F\A{i}]\cdot \Prob[F\A{i}]+\Exp[\MM\mid F\A{n}]\cdot \Prob[F\A{n}]\\
%\leq & \sum_{i=2}^{n-1}\Exp[\MM\mid F\A{i}]\cdot \Prob[F\A{i}]+\frac{\epsilon}{n^2}\bigl(\,\Exp[\MM\mid F\A{n}]\cdot \Prob[F\A{n}]+\Exp[\MM\mid F\A{n-1}]\cdot \Prob[F\A{n-1}]\,\bigr)\\
%\leq & \sum_{i=2}^{n-1}\Exp[\MM\mid F\A{i}]\cdot \Prob[F\A{i}]+ \frac{\epsilon}{n^2} \cdot \sum_{i=2}^{n-1}\Exp[\MM\mid F\A{i}]\cdot \Prob[F\A{i}]\\
%\leq & (1+\frac{\epsilon}{n^2})(1-\frac{1}{n-1})\epsilon \cdot (\Exp[\MM\mid F\A{0}] \cdot \Prob[F\A{0}]+ \Exp[\MM\mid F\langle 1\rangle]\cdot \Prob[F\A{1}])~(induction)\\
%\leq & (1-\frac{1}{n})\epsilon \cdot (\Exp[\MM\mid F\A{0}] \cdot \Prob[F\A{0}]+ \Exp[\MM\mid F\langle 1\rangle]\cdot \Prob[F\A{1}])
%\end{align*}
Now, we prove the claim. Again, we rewrite the LHS as
$$
\Exp[\MM\mid \calF\A{i+1}]\cdot \Prob[\calF\A{i+1}]
=\sum_{|S|=i+1} \sum_{F_S} \sum_{H_{\bS}}
\Bigl(\,
\Prob[ F_S,  H_{\bS}]\cdot
\MM(F_S, H_{\bS})\,\Bigr).
$$
%Here $ H_{\bS}$ means for each $s\in \bS, s\realize \textcircled{s}$. \\
Similarly, we have the RHS to be
$$
\Exp[\MM\mid \calF\A{i}]\cdot \Prob[\calF\A{i}]
=\sum_{|S'|=i} \sum_{F_{S'}} \sum_{H_{\bS'}}
\Bigl(\,
\Prob[ F_{S'},  H_{\bS'}]\cdot
\MM(F_{S'}, H_{\bS'})\,\Bigr) \text{ and }
$$
$$
\Exp[\MM\mid \calF\A{i-1}]\cdot \Prob[\calF\A{i-1}]
=\sum_{|S^{''}|=i-1} \sum_{F_{S^{''}}} \sum_{H_{\bS''}}
\Bigl(\,
\Prob[F_{S^{''}},  H_{\bar{S^{''}}}]\cdot
\MM(F_{S^{''}}, H_{\bar{S^{''}}})\,\Bigr).
$$
Let $C(F_S, H_{\bS})=
\Prob[ F_S,  H_{\bS}]\cdot \MM(F_S, H_{\bS})$.
Think all $(F_{S'},H_{\bS'})$ with $|S^{'}|=i$
and all $(F_{S''},H_{\bS''})$ with $|S^{''}|=i-1$
as buyers.
The buyers want to buy all terms in LHS.
The budget of buyer $(F_{S'},H_{\bS'})$ is $C(F_{S'},H_{\bS'})$.
We show there is a charging scheme such that
every term $C(F_{S}, H_{\bS})$ is fully paid by the buyers and
each buyer spends at most an $\frac{\e}{6}$ fraction of her budget.

Suppose we are selling the term $C(F_S, H_{\bS})$.
Consider the following charging scheme.
Suppose $v\in S$ the node that realizes to point $f\in F_S$
which is the closest point to $H_{\bS}$ in $F_S$.
Suppose $t\in S$ the node that is realized to point $F_t\in F_S$
which is the second closest point to $H_{\bS}$ in $F_S$.
Let $S'=S\setminus \{v_1\}$, $S''=S'\setminus \{v_2\}$.
If $(F_{S'}, R_{\bS'})$ is obtained from $(F_S, H_{\bS})$ by sending $v_1$ to
a point in its home $\Home(v_1)$,
we say $(F_{S'}, R_{\bS'})$
is consistent with  $(F_{S}, R_{\bS})$,
denoted as $(F_{S'}, R_{\bS'})\consistent (F_{S}, R_{\bS})$.
If $(F_{S''}, R_{\bS''})$ is obtained from $(F_{S'}, H_{\bS'})$ by sending $v_2$ to
a point in its home $\Home(v_2)$,
we say $(F_{S''}, R_{\bS''})$
is consistent with  $(F_{S'}, R_{\bS'})$,
denoted as $(F_{S'}, R_{\bS'})\consistent (F_{S}, R_{\bS})$.
Let
$$
Z(F_{S}, H_{\bS})=
\sum_{(F_{S'}, H_{\bS'})\consistent (F_{S}, H_{\bS})} \Prob[(F_{S'}, H_{\bS'})],
\quad\text { and }$$
$$
Z(F_{S'}, H_{\bS'})=
\sum_{(F_{S''}, H_{\bS''})\consistent (F_{S'}, H_{\bS'})} \Prob[F_{S''}, H_{\bS''}]
$$
Now, we claim that for any fixed $(F_{S''}, H_{\bS''})$,
$$
 \sum_{(F_{S'}, H_{\bS'})\consistent (F_{S''}, H_{\bS''})} \frac{\Prob[F_{S'},  H_{\bS'}]}
{Z(F_{S'}, H_{\bS'})}
\leq
\sum_{v\in \bS''} \frac{\Prob[v\notin \Home(v)]}{\Prob[v\in \Home(v)]}.
$$
The proof of the claim is essentially the same as
Lemma~\ref{lm:mstcharge}.
We first observe that the denominators of all terms are in fact the same,
by the definition of $Z$.
Then, the proof can be completed by canceling out the same multiplicative terms from the numerators and the denominator.


Now, we specify how to charge each buyer.
For each buyer $(F_{S'},H_{\bS'})\sim (F_{S}, H_{\bS})$,
we charge $(F_{S'}, H_{\bS'})$ the following amount of money
$$
2(m+2) \Prob[ F_S,  H_{\bS}] \MM(F_{S'}, H_{\bS'})\cdot
\frac{\Prob[F_{S'},  H_{\bS'}]}
{Z(F_{S}, H_{\bS})},
$$
and we charge every buyer $(F_{S''}, H_{\bS''})$ consistent with $(F_{S'}, H_{\bS'})$ the following amount of money
\begin{align*}
%&\frac{\Prob[F_{S'}, H_{\bS'}]}
%{Z(F_{S}, H_{\bS})}\cdot \frac{\Prob[F_{S''},  H_{\bS''}]}
%{Z(F_{S'}, H_{\bS'})}
%\Prob[ F_S,  H_{\bS}]\cdot 2(n+2)\MM(F_{S''}, H_{\bS''})\\
2(m+2) \Prob[ F_S'',  H_{\bS''}] \MM(F_{S''}, H_{\bS''})
\cdot
\frac{\Prob[F_{S}, H_{\bS}]}
{Z(F_{S}, H_{\bS})}\cdot \frac{\Prob[F_{S'},  H_{\bS'}]}
{Z(F_{S'}, H_{\bS'})}.
\end{align*}
In this case, we say $(F_{S''}, H_{\bS''})$ is a {\em sub-buyer} of the term $C(F_S, H_{\bS})$.
By Lemma~\ref{lm:del1or2}, we can see that $A(F_S, H_{\bS})$ is fully paid.
To prove the claim,
it suffices to show that each buyer $(F_{S'}, H_{\bS'})$ and each sub-buyer $(F_{S''}, H_{\bS''})$
has been charged at most $\frac{\epsilon}{6}A(F_{S'}, H_{\bS'})$ dollars.
By the above charging scheme,
the terms in LHS that are charged to buyer $(F_{S'}, H_{\bS'})$
are consistent with $(F_{S'}, H_{\bS'})$.
Using the same argument as in Lemma~\ref{lm:mstcharge},
we can show the spending of $(F_{S'}, H_{\bS'})$ as a buyer
is at most
$$\frac{\epsilon}{nm}\cdot \MM(F_{S'}, H_{\bS'})\cdot \Prob[F_{S'},  H_{\bS'}].$$

For notational convenience, we let
$B= 2(m+2)  \MM(F_{S''}, H_{\bS''})\Prob[ F_{S''},  H_{\bS''}]$.
The spending of $(F_{S''}, H_{\bS''})$ as a sub-buyer can be bounded as follows:
\begin{align*}
&B
\cdot\sum_{(F_{S'}, H_{\bS'})\consistent (F_{S''}, H_{\bS''})}
\sum_{(F_{S}, H_{\bS})\consistent (F_{S'}, H_{\bS'})}
\left(\,
\frac{\Prob[F_{S}, H_{\bS}]}{Z(F_{S}, H_{\bS})}\cdot
\frac{\Prob[F_{S'},  H_{\bS'}]} {Z(F_{S'}, H_{\bS'})}
\,\right)\\
\leq &\,B\cdot
 \sum_{(F_{S'}, H_{\bS'})\consistent (F_{S''}, H_{\bS''})}
 \sum_{(F_{S}, H_{\bS})\consistent (F_{S'}, H_{\bS'})}
  \frac{\Prob[F_{S'},  H_{\bS'}]}
{Z(F_{S'}, H_{\bS'})} \\
\leq & B\cdot
 mn \cdot
 \sum_{(F_{S'}, H_{\bS'})\consistent (F_{S''}, H_{\bS''})} \frac{\Prob[F_{S'},  H_{\bS'}]}
{Z(F_{S'}, H_{\bS'})} \\
\leq &\, B\cdot mn \cdot
\sum_{v\in \bS''} \frac{\Prob[v\notin \Home(v)]}{\Prob[v\in \Home(v)]} \\
\leq &\, \frac{\e}{6}\cdot \MM(F_{S''}, H_{\bS''}) \cdot \Prob[F_{S''},  H_{\bS''}]
\end{align*}
%To see the second and the third inequality,
%for a fixed vertex $v$, consider the quantity
%$$
%\sum_{(F_{S'}, H_{\bar{S}'})\consistent (F_{S''}, H_{\bar{S}''}), S''=S'\setminus \{v\}}
%\frac{\Prob[F_{S'}, H_{\bar{S}'}]}{Z(F_{S'}, H_{\bar{S}'})}
%$$
%By the definition of $Z$, we can see that denominators of all terms are in fact the same.
%Then it is not hard to see the quantity is at most $\frac{\Prob[v\notin \Home(v)]}{\Prob[v\in \Home(v)]}$.
In the first inequality, we use the fact that $\frac{\Prob[F_{S}, H_{\bS}]}{Z(F_{S}, H_{\bS})}\leq 1$.
Note that for each $(F_{S'}, H_{\bar{S}'})$, there are at most $mn$ different $(F_{S}, H_{\bar{S}})$
such that $(F_{S}, H_{\bar{S}})\consistent (F_{S'}, H_{\bar{S}'})$. So we have the second inequality.
This completes the proof of the lemma.
\qed
\end{proof}





==> app-warmup.tex <==
\section{Estimating $k$th Closest Pair in the Existential Uncertainty Model}
\label{app:CP}

Again, we construct the HPF $\hpf$.
Let the random variable $Y$ be the largest integer $i$ such that there are at least $k$ point collisions in $\Gamma_i$.
Here we use a point collision to denote that a pair of points are present in the same component.
Note that if there are exactly $i$ points in a component, the amount of point collisions in this component is ${i\choose 2}$.
We denote as $\Gamma\A{\#j}$ the event that there are exactly $j$ point collisions among the partition $\Gamma$ on $\P$. Similarly, we can rewrite $\Exp[\KCP]$ by $\Exp[\KCP]=\sum_{i=1}^{m-1} \Prob[Y=i]\Exp[\KCP\mid Y=i]$.

We use dynamic programming technique to achieve an $\FA$ for computing $\Exp[\KCP]$.
Note that conditioning on $Y=i$, the value of $\KCP$ is between $\dist(e_{i})$ and $m\cdot \dist(e_{i})$. So we only need to show the following lemma.

\begin{lemma}
\label{lm:samCP_k}
We can compute $\Prob[Y=i]$ in polynomial time. Moreover, there exists a polynomial time sampler conditioning on $Y=i$.
\end{lemma}

\begin{proof}
We denote $E[a,b]$ ($1\leq a\leq i-1$, $b\leq k$) the event that among the first $a$ components in $\Gamma'_i $, there are exactly $b\leq k$ point collisions. We denote the probability of $E[a,b]$ by $\Prob[a,b]$. We give the dynamic programming as follows.

\begin{enumerate}
\item If $\sum_{1\leq j\leq a}{|C_{j}|\choose 2} < b$, $\Prob[a,b]=0$. If $b = 0$, $\Prob[a,b]=\prod_{1\leq j\leq a}\Prob[C_j\A{\leq 1}]$. If $b<0$, $\Prob[a,b]=0$.
\item If $\sum_{1\leq j\leq a}{|C_{j}|\choose 2} \geq b$, $1\leq b\leq k$, $\Prob[a,b]=\sum_{0\leq l\leq n_{a}} \Prob[C_{a}\A{l}]\cdot \Prob[a-1,b-{l\choose 2}]$.
\end{enumerate}
\noindent
By the above dynamic programming, we can compute $\Prob[i-1,l]$ for $0\leq l\leq k-1$ in polynomial time. \\
By the definition of $Y=i$, it is no hard to see that we can rewrite $\Prob[Y=i]$ as follows:
$$
\Prob[Y=i]=\sum_{1\leq n_1\leq |\mu'_{i+1}|, 1\leq n_2\leq |\mu''_{i+1}|} \Prob[\mu'_{i+1}\A{n_1}]\cdot \Prob[\mu''_{i+1}\A{n_2}]\cdot
\left( \sum_{k-{n_1+n_2\choose 2}\leq l\leq k-1-{n_1\choose 2}-{n_2\choose 2}} \Prob[\Gamma'_i\A{\#l}]\right)
$$
Note that we can compute $\Prob[Y=i]$ in polynomial time. We need to describe our sampler conditioning on $Y=i$. We first sample the event $\mu'_{i+1}\A{n_1}\wedge \mu''_{i+1}\A{n_2}$ with probability $\Prob[\mu'_{i+1}\A{n_1}\wedge \mu''_{i+1}\A{n_2}\mid Y=i]$. Then conditioning on $k-{n_1+n_2\choose 2}\leq l\leq k-1-{n_1\choose 2}-{n_2\choose 2}$, we sample the total number of point collisions in $\Gamma'_i$. Then we sample the number of present points in each component in $\Gamma'_i$ using the dynamic programming. Finally, based on the number of present points in each component, we sample the present points by Lemma~\ref{lm:samTj}. \\
Using the Monte Carlo method, we only need to take $O(\frac{m}{\e^2}\ln m)$ independent samples for estimating $\Exp[\KCP\mid Y=i]$. Thus, we totally take $O(\frac{m^2}{\e^2}\ln m)$ independent samples.
\qed
\end{proof}

\begin{theorem}
\label{thm:kcp}
There is an FPRAS for estimating the expected distance between
the $k$th closest pair in the existential uncertainty model.
\end{theorem}



==> app.tex <==
\section{Estimating $\Prob[\CP\leq 1]$ in the locational uncertainty model}
\label{app:CP}

\linesnumbered
\begin{algorithm}[t]
\caption{Estimating $\Pr[\CP\leq 1]$}
\label{algo:cp}
\KwSty{\core:} $\H=\{s_i\mid p_i\geq \frac{\e}{m^3}\}$. Set $\calF=\P\setminus \H$.\\
Estimate $\Prob[\calF\A{0} \wedge \CP\leq 1]$:
Take $N_0=O((m/\e)^{4})$ independent samples. Suppose $M_0$ is the number of samples satisfying $\CP\leq 1$ and $\calF\A{0}$.
$T_0\leftarrow \frac{M_0}{N_0}$. \\
Estimate $\Prob[\calF\A{1} \wedge \CP\leq 1]$: For each point $s_i\in \calF$, take $N_1=O((m/\e)^{4})$ independent samples conditioning on the event $\calF\A{\{s_i\}}$. Suppose there are $M_i$ samples satisfying $\CP\leq 1$.
$T_1\leftarrow \sum_{s_i\in \calF}p_iM_i/N_1$.\\
Estimate $\Prob[\calF\A{2} \wedge \CP\leq 1]$: For each point pair $s_i,s_j\in \calF$, take $N_2=O((m/\e)^{4})$ independent samples conditioning on the event
$\calF\A{\{s_i,s_j\}}$. Suppose there are $M_{ij}$ samples satisfying $\CP\leq 1$.
$T_2\leftarrow \sum_{s_i,s_j \in \calF}p_i p_jM_{ij}/N_2$.\\
\KwSty{Output:} $T_0+T_1+T_2$
%\end{algorithmic}
\end{algorithm}


The approximation algorithm for the {\em locational uncertainty model} is similar to the one in the {\em existence uncertainty model}. Here we just briefly describe the algorithm without many details.
We denote the set of nodes as $\V=\{v_1,\ldots, v_n\}$
and the set of points $\P=\{s_1, \ldots, s_m\}$,
where $n=|\V|$ and $m=|\P|$. We use the notation $v \realize s$ to denote the event that
node $v$ is present at point $s$ and let $\p_{vs}=\Prob[v \realize s]$. For each point $s\in \P$, we denote the probability that there exists some node $v\realize s$ as $\Prob[\realize s]$. For a point subset $H\in \P$, we denote the probability that there exists some node $u\realize s$ for any $s\in H$ as $\Prob[\realize H]$.
Assume that the distribution of the location of each node is discrete. Let $H\A{i}$ to denote the event that exactly $i$ nodes are in a point set $H$.

We construct the \core\ $\H$ where each point $s$ in $\H$ has no negligible probability to be located by some nodes, i.e, $\Prob[\realize s]\geq \frac{\epsilon}{nm}$. Let $\calF=\P\setminus \H$. Then we could rewrite $\Prob[\CP \leq 1]$ by $\sum_{0\leq i\leq n}\Prob[\calF\A{i}\wedge \CP \leq 1]$. Still the contribution of the term $\sum_{3\leq i\leq n}\Prob[\calF\A{i}\wedge \CP \leq 1]$ are negligible. So we only need to estimate the first three terms.

If for any two points $s,t\in \H$ with $\dist(s,t)\leq 1$, we have $\Prob[\realize s,t]\leq \frac{\epsilon^3}{(nm)^4}$. We can simply use $\sum_{(s,t):s,t\in \H, \dist(s,t)\leq 1}\Prob[\realize s,t]$ to estimate $\Prob[\calF\A{0}\wedge \CP\leq 1]$ by Inclusion-exclusion principle and the following lemma.

\begin{lemma}
\label{lm:estCPlocational}
For 3 points $s_1,s_2,s_3\in \P$, if $\p_i=\Prob[\realize s_i]\geq \frac{\epsilon}{(nm)^2}$ for $i=1,2,3$, and $\p_{1,2}=\Prob[\realize s_1,s_2]\leq \frac{\epsilon^2}{(nm)^4}$, $\p_{2,3}=\Prob[\realize s_2,s_3]\leq \frac{\epsilon^3}{(nm)^4}$. We have $\p_{1,2,3}=\Prob[\realize s_1,s_2,s_3]\leq \frac{3\epsilon}{nm}\cdot \min\{\p_{1,2},\p_{2,3}\}$.
\end{lemma}
\begin{proof}
Note that there is a node $v\in \V$ with probabilities $\p_{v s_i}\geq (1-\frac{\epsilon}{nm})\p_i$ for $i=1,2,3$. Or else, $\p_{1,2}$ or $\p_{2,3}$ could not be bounded as the condition. Then we have
$$\p_{1,2,3}\leq \Prob[\realize s_1,s_2 \mid t\nvDash s_1 \wedge t\nvDash s_2]+\Prob[\realize s_1,s_2,s_3 \mid t\realize s_1 \vee t\realize s_2]\leq \frac{2\epsilon\p_{1,2}}{nm}+\frac{\epsilon\p_{1,2}}{nm}=\frac{3\epsilon\p_{1,2}}{nm}$$
Similarly, we have $\p_{1,2,3}\leq \frac{3\epsilon\p_{2,3}}{nm}$.
\qed
\end{proof}

If there are two points $s,t\in \H$ with $\dist(s,t)\leq 1$ such that $\Prob[\realize s,t]\geq \frac{\epsilon^3}{(nm)^4}$, we can estimate $\Prob[\calF\A{0}\wedge \CP\leq 1]$ by sampling.
For $\Prob[\calF\A{1}\wedge \CP \leq 1]$, we rewrite it by $\sum_{v\in \V, s\in \calF}p_{vs}\cdot \Prob[\calF\A{1}\wedge \CP \leq 1 \wedge v\realize s]$. For a certain poit $s\in \calF$, if there is no point $t\in \H$ such that $\dist(s,t)\leq 1$, we have $\Prob[\calF\A{1}\wedge \CP \leq 1 \wedge v\realize s]=\p_{vs}\cdot \Prob[\calF\A{0}\wedge \CP\leq 1]$. Otherwise, we use the Monte Carlo method with enough samples conditioning on the event $\calF\A{1}\wedge v\realize s$ for each pair $(v,s)$, and achieve a poly-bounded estimation for $\Prob[\calF\A{1}\wedge \CP \leq 1 \wedge v\realize s]$.
Similarly, we could estimate the third term and achieve an FPRAS for $\Prob[\CP\leq 1]$ in the {\em locational uncertainty model}.

\eat{
\section{Estimating $\Exp[\CP]$ in the locational uncertainty model}
\label{app:ECP}
In the locational uncertainty model, we use the term {\em nodes} to refer to the vertices $\V$ of the spanning tree
and {\em points} the points in the metric space $\P$.
We have $|\V|=n$ and $|\P|=m$. Let $H\A{i}$ to denote the event that exactly $i$ nodes are in a point set $H$. For any node $v\in \V$ and point $s\in \P$,
we use the notation $v \realize s$ to denote the event that
node $v$ is present at point $s$.
Let $\p_{vs}=\Prob[v \realize s]$, i.e., the probability that node $v$ is present at point $s$. Similarly, we define $H\A{\leq i}$ and $\calT_i\A{\leq 1}$.
Our technique is very close to under the existential uncertainty model. Based on $\P$, we still construct an HDT. $L_i$ still represents that the event $T^*_{i,1}\A{1} \wedge T^*_{i,2}\A{1} \wedge \calT_i\A{\leq 1}$, i.e, there exists a node $u$ located to $T^*_{i,1}$ and a node $v$ located to $T^*_{i,2}$, and the rest nodes locate to different components in $\calT_{i}$. Then we can rewrite $\Exp[\CP]$ by $\Exp[\CP]=\sum_{i=1}^{m-1} \Prob[L_i]\Exp[\CP\mid L_i]$. Note that each node has a personal probability distribution present in components $T^*_{i,1}\cup T^*_{i,2}\cup \calT_i$. If a node $u$ is already present in a component $T$, we simply realize $u$ to point $s\in T$ with probability $\frac{\Prob[p_{us}]}{\Prob[p_{uT}]}$. Here $p_{uT}$ represents the probability that node $u$ is present in component $T$. Then we only need to how to compute $\Prob[L_i]$ and how to sample nodes into different components including $T^*_{i,1}$ and $T^*_{i,2}$. We have the following theorem:

\begin{theorem}
\label{thm:jerrum2004permanent}
(~\cite{jerrum2004permanent})
There exists a fully polynomial almost uniform sampler for perfect matchings in an arbitrary nonnegative weighted bipartite graph and an $\FA$ for computing permanent (counting perfect matchings).
\end{theorem}

We first add $m-i-n+1$ (to make the number of nodes equal to the components in $\calT_{i}$) nodes with equal probability $\frac{1}{m-i-1}$ locating to each component in $\calT_{i}$. Note that a perfect matching between nodes and components $T^*_{i,1}\cup T^*_{i,2}\cup \calT_i$ now exactly corresponds to a sample which assigns nodes into different components including $T^*_{i,1}$ and $T^*_{i,2}$ in the original graph. Then we could apply Theorem~\ref{thm:jerrum2004permanent} to achieve a polynomial almost uniform sampler and approximately compute $\Prob[L_i]$ (suppose the permanent in the new graph is $A_i$, we have $\Prob[L_i]=\frac{(m-i-1)^{(m-i-n+1)}}{(m-i-n+1)!}\cdot A_i$). Above all, we could produces a $(1\pm\epsilon)$-estimate for $\Exp[\CP]$ in the locational uncertainty model. Combine the results in the existential and locational uncertainty model, we obtain the main result Theorem~\ref{thm:cp}.\\
}

\section{NP-hardness of Computing $\Exp[\CP]$}
\label{app:npcp}
\begin{theorem} Computing $\Exp[\CP]$ under the  existential uncertainty model is NP-hard.
\end{theorem}
\begin{proof}
We only need to show that $\Prob[\CP]\leq_{p} \Exp[\CP]$, i.e., to give a reduction from $\Prob[\CP]$ to $\Exp[\CP]$.

Let the given sample be $M$. Assume the distance between the farthest pair in $\P$ is $D$ ( we do not consider $D$ appears in more than 1 pair, cause that situation is not hard to deal with ), we slightly change $M$ to $M'$ by decreasing the distance between the farthest pair by an enough small parameter $\delta$ (the distance maintains farthest). We have $\Prob[\CP=D]=\frac{\Exp[\CP(M)]-\Exp[\CP(M')]}{\delta}$. Using the same way, we could compute $\Prob[\CP=l]$ for $l$ which is the distance between a certain pair. Then it is easy to compute $\Prob[\CP]$. By reduction, $\Exp[\CP]$ is NP-hard.
\qed
\end{proof}

\section{Another FPRAS for MST}
\label{app:mst}
W.l.o.g., we assume that for each point, there is only one node that may realize
to this point.
Our algorithm is a slight generalization of
the one proposed in \cite{kamousi2011stochastic}.
Let $\Exp[i]$ be the expected $\MST$ length conditioned on the event that
all nodes $\{s_1,\ldots,s_n\}$ are realized to points in $\{u_i,\ldots, u_m\}$
(denote the event by $\iin(i,m)$).
Let $\Exp'[i]$ be the expected $\MST$ length conditioned on the event that
all nodes $\{s_1,\ldots,s_n\}$ are realized to $\{u_i,\ldots, u_m\}$
and at least one node is realized to $u_i$.
We use $s\realize u$ to denote the event that node $s$ is realized to point $u$.
It is easy to see that
\begin{align*}
\Exp[i]=\Exp'[i]\Prob[\exists s, s\realize u_i\mid \iin(i,m)]+
\Exp[i+1]\Prob[\not\exists s, s\realize u_i\mid \iin(i,m)]
\end{align*}

For a particular point $u_i$,
we reorder the points $\{u_i,\ldots, u_m\}$ as $\{u_i=r_i,\ldots, r_m\}$ in increasing order of distance from $u_i$.
Let $\Exp'[i, j]$ be the expected $\MST$ length for all nodes
conditioned on the event that
all nodes are realized to $\{r_i,\ldots, r_j\}$ (denoted as $\iin'(i,j)$) and
$\exists s, s\realize u_i$.
Let $\Exp''[i, j]$ be the expected $\MST$ length for all nodes
conditioned on the event $\iin'(i,j) \wedge
(\exists s, s\realize u_i)\wedge (\exists s', s'\realize r_j)$.
We can see that
\begin{align*}
\Exp'[i,j]=&\Exp''[i,j]\Prob[\exists s', s'\realize u_j\mid \iin'(i,j), \exists s, s\realize u_i] \\
&+ \Exp'[i,j-1]\Prob[\not\exists s, s\realize u_i\mid \iin'(i,j), \exists s, s\realize u_i]
\end{align*}
It is not difficult to see the probability
$\Prob[\exists s', s'\realize u_j\mid \iin'(i,j), \exists s, s\realize u_i]$
can be computed in polynomial time.
Here we use the assumption that for each point, only one node that may realize to it.
Moreover, we can also take samples conditioning on event
$\iin'(i,j) \wedge (\exists s, s\realize u_i)\wedge (\exists s', s'\realize r_j)$.
Therefore $\Exp''[i,j]$ can be approximated within a factor of $(1\pm \epsilon)$ using
the Monte Carlo method in polynomial time since it is a nice instance.
The number of samples needed can be bounded by a polynomial.
%$O(\frac{nm^2}{\epsilon^2}(\log m+\log n))$.

We can easily generalize the above algorithm to the case where
$\sum_{j=1}^m p_{ij}\leq 1$, i.e., node $i$ may not be present with some probability.
Indeed, this can be done by generalizing the definition of
$\iin(i,j)$ (and similarly $\iin'(i,j)$)
to be the event that each nodes is either not
present or realized to some node in $\{r_i,\ldots, r_j\}$.


\section{MST}


\vspace{0.2cm}
\linesnotnumbered
\begin{algorithm}[t]
\caption{Estimating $\Exp[\MST]$}

\label{alg:estMST}
\KwSty{-- Procedure 1: Finding the \core\ $\H$ } \\
\nl Among all points $r$ with $p(r)\geq \frac{\epsilon}{16m}$, find the furthest two points $s$ and $t$.\\
\nl Set $\H\leftarrow\B(s, \dist(s,t))$, which is the ball
centered at $s$ with radius $\dist(s,t)$.\\
\KwSty{-- Procedure 2: Estimating $\Exp[\,\MST\mid \calF\A{0} \,] \cdot \Prob[ \calF\A{0}]$} \\
\nl Take $N_0=O(\frac{nm^2}{\e^4}\ln n)$ random samples. Set $A\leftarrow \emptyset$ at the beginning.\\
\nl For each sample $G_i$, if it satisfies $\calF\A{0}$, $A\leftarrow A\cup \{G_i\}$.\\
\nl $T_0\leftarrow \frac{1}{N_0}\sum_{G_i\in A}\MST(G_i)$.\\
\KwSty{-- Procedure 3: Estimating $\Exp[\,\MST\mid \calF\A{1} \,] \cdot \Prob[ \calF\A{1}]$}\\
\nl Set $B\leftarrow \{s\mid s\in \calF, \dist(s,\H)<\frac{n}{\e } \cdot \diam(\H)\}$. 2 Let $\Cl(v)$ be the event that $v$ is the only node that realizes to some node $s\notin \H$ and $s\in B$.\\
\nl Conditioning on $\Cl(v)$,
take $N_2=O\bigl( \frac{nm^2}{\e^{5}}\ln n\bigr)$ independent samples.
Let $A_v\leftarrow \{G_{v,i}\mid 1\leq i\leq N_1\}$ be the set of $N_1$ samples for $\Cl(v)$.\\
\nl $T_v\leftarrow \frac{1}{N_1}\sum_{G_{v,i}\in A_v}\MST(G_{v,i})$  ~~~~(estimating $\Exp[\,\MST\mid \Cl(v)]$)\\
\nl $T_1\leftarrow \sum_{v\in \V}\Bigl(\Prob[\Cl(v)]T_v+\sum_{s\in \calF\setminus B}\Prob[\calF\A{v}\wedge v\realize s]\,\dist(s,\H)\,\Bigr)$.\\
\nl \KwSty{Output:} $T_0+T_1$
\end{algorithm}


We need the following simple lemma. The proof of the first lemma is in Appendix.
\begin{lemma}
\label{lm:lmprob}
Consider two points $s$ and $t$ in $\P$. Suppose $p(s)\geq \delta$, $p(t)\geq \delta$ (Here $\delta \ll 0.2$ is a positive real number).
Suppose no node contributes to more than one half of both $p(s)$ and $p(t)$
(i.e., $\not\exists v\in V, \text{ s.t. }p_{vs}\geq 0.5 p(s)\text{ and } p_{vt}\geq 0.5 p(t)$).
Then, we have that $\Prob[\exists (v,u), v\ne u, v\realize s, u\realize t] = \Omega( \delta^2).$
\end{lemma}



\eat{
\begin{proof}
We only give a brief proof here. The details are in Appendix. Lemma~\ref{lm:est1MST} simply comes from the property of $\H$ and the Monte Carlo method. To prove Lemma~\ref{lm:est2MST}, we first rewrite the second term as follows:
\begin{align*}
\Exp[\,\MST\mid \calF\A{1} \,]\cdot \Prob[\calF\A{1}]
%&=\sum_{v\in \V} \Exp[\,\MST\mid F\A{v} \,]\,\Prob[ F\A{v}]
=\sum_{v\in \V} \Bigl(\,\sum_{s\in \calF} \Prob[\calF\A{v}\wedge v\realize s]\, \Exp[\,\MST\mid \calF\A{v}, v\realize s ]\,\Bigr)
\end{align*}
Fix a node $v$. To estimate $\sum_{s\in \calF} \Prob[\calF\A{v}\wedge v\realize s]\, \Exp[\MST\mid \calF\A{v}, v\realize s ]$, we consider the following two situations:
\begin{enumerate}
\item
Point $s\in B$, i,e, $\dist(s,\H)<\frac{n}{\e } \cdot \diam(\H)$. We estimate the sum for all $s\in B$. Notice that the sum is in fact $\Prob[\Cl(v)]\cdot\E[\,\MST\mid \Cl(v) ]$. Consider the size relationship between $\E[\,\MST\mid \Cl(v) ]$ and $\frac{1}{2}\Exp[\,\MST \mid \H\A{n}]$, we conclude that either the estimation is poly-bounded or the total contribution of $\Prob[\Cl(v)]\cdot\E[\,\MST\mid \Cl(v) ]$ is negligible.
\item
Point $s\in \calF\setminus B$.
We just use $\dist(s,\H)$
as the estimation of $\Exp[\MST\mid \calF\A{v}, v\realize s ]$.
\end{enumerate}
\qed
\end{proof}
}

We need some notations first.
Suppose $S$ is the set of nodes out of \core\ $\H$.
We use $\calF_S$ to denote the set of all possible realizations of all nodes in $S$ to points in $\calF$
(we can think of each element in $\calF_S$ as a $|S|$-dimensional vector where each coordinate
is indexed by a node in $S$ and its value is a point in $\calF$).
Similarly, we denote the set of realizations of $\bS=V\setminus S$ to points in $\H$ by $\calH_{\bS}$.
For any $F_S\in \calF_S$ and $H_{\bS}\in \calH_{\bS}$, we use $(F_S, H_{\bS})$ to denote the event that
both $F_S$ and $H_{\bS}$ happen
and $\MST(F_S, H_{\bS})$ to denote the length of the minimum spanning tree
under the realization $(F_S, H_{\bS})$.
We need the following combinatorial fact.

\begin{lemma}
\label{lm:mstchange}
Consider a particular realization $(F_S,H_{\bS})$,
where $S$ is the set of nodes not in $\H$.
$|S|\geq 2$. Let $d=\dist(v_S,u_S)=\min_{v\in S,u\in \bS}\{\dist(u,v)\}$ where $v_S\in F_S$, $u_S\in H_{\bS}$.
The realization $(F'_{S'}, H'_{\bS'})$ is obtained from $(F_S,H_{\bS})$
by sending the node $v_S$ to $\H$, where $S'=S\setminus{v_S}$.
Then $\MST(F_S, H_{\bS})\leq 4\MST(F'_{S'}, H'_{\bS'})$.
\end{lemma}

\begin{proof}
We have
$$
4\MST(F'_{S'},H'_{\bS'})\geq 2\MST(F'_{S'},H'_{\bS'})+2d\geq \MST(F'_{S'},H_{\bS})+2d\geq \MST(F_S,H_{\bS})
$$
The second inequality holds since the length of the minimum spanning tree is at most two times
the length of the minimum Steiner tree (We think $\MST(F'_{S'},H_{\bS})$ as a Steiner tree
connecting all nodes in $F_{S'}\cup H_{\bS}$).
\qed
\end{proof}

The only remaining part for establishing Theorem~\ref{thm:mst}
is to prove the following essential lemma, via a careful charging argument.
\begin{lemma}
\label{lm:mstcharge}
For any $\epsilon>0$,
if $\H$ satisfies the properties in Lemma~\ref{lm:home}, we have that
$$
\sum_{i>1}\Exp[\,\MST\mid \calF\A{i}]\cdot \Prob[\calF\A{i}]\leq \epsilon\cdot\Exp[\,\MST\mid \calF\langle 1\rangle]\cdot \Prob[\calF\A{1}].
$$
\end{lemma}

\begin{theorem}
\label{thm:mst}
There is an FPRAS for estimating the expected length of
the minimum spanning tree in the locational uncertainty model.
\end{theorem}



\section{Proof of Lemma \ref{lm:lmprob}}

\begin{proof}
Note that we only need to show the correctness while $p(s)=p(t)=\delta$. According to the given conditions, we have that
$$
\frac{p_{vs}p_{vt}}{p(s)p(t)}\leq \frac{1}{4}\Bigl(\frac{p_{vs}}{p(s)}+\frac{p_{vt}}{p(t)}\Bigr)^2\leq \frac{3}{8}\Bigl(\frac{p_{vs}}{p(s)}+\frac{p_{vt}}{p(t)}\Bigr)
$$
Then, we can see that
\begin{align*}
&\Prob[\exists (v,u), v\neq u, v\realize s, u\realize t] = 1-\Pi_{v\in V}(1-p_{vs})-\Pi_{v\in V}(1-p_{vt})+\Pi_{v\in V}(1-p_{vs}-p_{vt}) \\
&= (1-\Pi_{v\in V}(1-p_{vs}))(1-\Pi_{v\in V}(1-p_{vt}))+\Pi_{v\in V}(1-p_{vs}-p_{vt})-\Pi_{v\in V}(1-p_{vs})(1-p_{vt})\\
&\geq (1-\Pi_{v\in V}(1-p_{vs}))(1-\Pi_{v\in V}(1-p_{vt}))-\sum_{v\in V}p_{vs}p_{vt} \\
&\geq (1-(1-\frac{p(s)}{n})^n)(1-(1-\frac{p(t)}{n})^n)-\sum_{v\in V}\frac{3}{8} p(s)p(t) \Bigl(\frac{p_{vs}}{p(s)}+\frac{p_{vt}}{p(t)}\Bigr) \\
&\geq (1-e^{-p(s)})(1-e^{-p(t)})-\frac{3}{4}p(s)p(t) \\
&\geq (0.9\delta)^2-\frac{3}{4}\delta^2 = 0.06\delta^2~~~(\delta\ll 0.2)
\end{align*}
\qed
\end{proof}

\section{Proof of Lemma \ref{lm:home}}

\begin{proof}
For each point $r$ that is not in $\H$, we know $p(r)<\frac{\epsilon}{16m}$.
Therefore, we have that
and  $p(\calP\setminus \H)<\frac{\epsilon}{16}$.
and  $p(\H)\geq n-\frac{\epsilon}{16}$.
Consider two cases:
\begin{enumerate}
\item There is no node $v\in V$ such that $p_{vs}\geq 0.5 p(s)\text{ and } p_{vt}\geq 0.5 p(t)$.
In this case, by Lemma~\ref{lm:lmprob}, we have that
$
\Exp[\MST\mid \H\A{n}]\geq \dist(s,t) \Prob[\exists (v,u), v\ne u, v\realize s, u\realize t]
\geq \Omega\Bigl(\dist(s,t) \frac{\epsilon^2}{m^2}\Bigr).
$
\item There is a node $v$ such that $p_{vs}\geq 0.5 p(s)\text{ and } p_{vt}\geq 0.5 p(t)$.
In this case, conditioning on the event that a different node $u$ is realized to an arbitrary point $q$
$
\Exp[\MST\mid \H\A{n}]\geq \dist(s,q) \Prob[v\realize s]+\dist(t,q) \Prob[v\realize t]
\geq \dist(s,t) \frac{\epsilon}{32m}.
$
\end{enumerate}
In either case, $\H$ satisfies both P1 and P2.
\qed
\end{proof}

\section{Proof of Lemma \ref{lm:est1MST}}
\begin{proof}
Due to (P2),
we have a nice instance and can therefore obtain a $(1\pm\epsilon)$-estimate for $\Exp[\,\MST\mid \H\A{n}\,]$
using the Monte Carlo method with $O(\frac{nm^2}{\e^4}\ln n)$ samples satisfying $\H\A{n}$ (by Lemma~\ref{lm:chernoff}).
By the first property of $\H$, with probability close to 1, a sample satisfies $\H\A{n}$.
So, the expected time to obtain an useful sample is bounded by a constant.
Overall, we can obtain a $(1\pm\epsilon)$-estimate of
the first term with using $N_1=O(\frac{nm^2}{\e^4}\ln n)$ samples with high probability.
\qed
\end{proof}

\section{Proof of Lemma \ref{lm:est2MST}}

\begin{proof}
To compute the second term, we first rewrite it as follows:
\begin{align*}
\Exp[\,\MST\mid \calF\A{1} \,]\cdot \Prob[\calF\A{1}]
%&=\sum_{v\in \V} \Exp[\,\MST\mid F\A{v} \,]\,\Prob[ F\A{v}]
=\sum_{v\in \V} \Bigl(\,\sum_{s\in F} \Prob[\calF\A{v}\wedge v\realize s]\, \Exp[\,\MST\mid \calF\A{v}, v\realize s ]\,\Bigr)
\end{align*}
%We can easily see that $\Prob[F\A{v}\wedge v\realize s]$ can be computed precisely in poly-time.
Fix a  node $v$.
To estimate $\sum_{s\in F} \Prob[\calF\A{v}\wedge v\realize s]\, \Exp[\MST\mid \calF\A{v}, v\realize s ]$, we consider the following two situations:
\begin{enumerate}
\item
Point $s\in B$, i,e, $\dist(s,\H)<\frac{n}{\e } \cdot \diam(\H)$.

We estimate the sum for all $s\in B$. Notice that the sum is in fact $\Prob[\Cl(v)]\cdot\E[\,\MST\mid \Cl(v) ]$.
%Here $v\realize \Cl(s)$ means that node $v$ is present at some point $s\in \Cl(s)$.
We can see that $\Prob[\Cl(v)]$ can be computed exactly in linear time.
We argue the quality of the estimation taken on $N_2=O\bigl( \frac{nm^2}{\e^{5}}\ln n\bigr)$ samples is good
by considering the following two cases:
%If
%$$\sum_{s:\dist(u,H)<n^{10}}\Exp[\,\MST \mid F\A{v}, v\realize s ]\cdot\Prob[v\realize s \mid F\A{v}]
%\geq \frac{1}{n^3}\Exp[\,\MST \mid H\A{n}]]\geq \frac{1}{(mn)^5}\diam(H),
%$$
    \begin{enumerate}
    \item Assume that $
    \E[\,\MST\mid \Cl(v) ]
    \geq \frac{1}{2}\Exp[\,\MST \mid \H\A{n}]\geq \Omega\Bigl(\frac{\e^2}{m^2}\Bigr)\diam(\H).
    $
    In this case, we have poly-bounded.
    This is because under the condition $\Cl(v)$,
    the maximum possible length of any minimum spanning tree is $O(\frac{n}{\e}\diam(\H))$.
    Hence we can use Monte Carlo to get a $(1\pm \epsilon)$-approximation
    of $\E[\,\MST\mid \Cl(v) ]$ with $O\bigl( \frac{nm^2}{\e^{5}}\ln n\bigr)$ samples.
    \item Otherwise, we assume that
    %$$
    %\Exp[\,\MST\mid F\A{1} ]\cdot \Prob[ H\A{1}]\leq \frac{1}{n^3} \Exp[\,\MST\mid H\A{n}]] \cdot \Prob[H\A{n}].
    %$$
    $
    \E[\,\MST\mid \Cl(v) ]
    \leq \frac{1}{2}\Exp[\,\MST \mid \H\A{n}]].
    $
    %Suppose we still use Monte Carlo to estimate $\E[\,\MST\mid F\A{v} \wedge v\realize s\wedge \Cl(s) ]$.
    The probability that the sample average is larger than $\Exp[\MST\mid \H\A{n}]] $
    is at most $\poly(\frac{1}{n})$ by Chernoff Bound. The probability that for all nodes $v$, the sample average are
    at most $\Exp[\MST\mid \H\A{n}]]$ is at least $1-\poly(\frac{1}{n})$ by union bound.
    If this is the case, we can see their total contribution
    to the final estimation of $\E[\MST]$ is less than $\e \Exp[\,\MST \mid \H\A{n}]] \Prob[\H\A{n}] $.
    In fact, this is because
    \begin{align*}
    & \sum_{v\in V} \Prob[\Cl(v)]\cdot\E[\,\MST\mid \Cl(v) ]\leq \sum_{v\in V}\Prob[\Cl(v)]\cdot \Exp[\,\MST \mid \H\A{n}]] \\
    & <\e \Exp[\,\MST \mid \H\A{n}]] \Prob[\H\A{n}].
    \end{align*}
    The second inequality is due to the fact that $\sum_{v\in V}\Prob[\Cl(v)]\leq n-p(\H)<\e/16<\e\Prob[\H\A{n}]$.
    \end{enumerate}
\item
Point $s\in \calF\setminus B$, each term has $\dist(s,\H)>\frac{n}{\e } \cdot \diam(\H)$.
We just use $\dist(s,\H)$
as the estimation of $\Exp[\MST\mid \calF\A{v}, v\realize s ]$.
This is because the length of $\MST$ is always at least $\dist(s,\H)$
and at most $\dist(s,\H)+n\cdot\diam(\H) \leq (1+\epsilon) \dist(s,\H)$.
\end{enumerate}
\qed
\end{proof}

\section{Proof of Lemma \ref{lm:mstcharge}}

\begin{proof}
We claim that for any $i>1$,
$
\Exp[\,\MST\mid \calF\A{i+1}]\cdot \Prob[\calF\A{i+1}]\leq \frac{\epsilon}{2}\Exp[\,\MST\mid \calF\langle i\rangle]\cdot \Prob[\calF\A{i}].
$
If the claim is true, then we can show the lemma easily by noticing that, for any $n\geq 2$,
%\begin{align*}
%\sum_{i> 1}\Exp[\,\MST\mid F\A{i}] \Prob[F\A{i}]
%\leq & \sum_{i=1}^{n-1}\Bigl(\frac{\epsilon}{2}\Bigr)^i  \Exp[\,\MST\mid F\langle 1\rangle] \Prob[F\A{1}]
%\leq  \epsilon\Exp[\,\MST\mid F\langle 1\rangle] \Prob[F\A{1}].
%\end{align*}
$
\sum_{i> 1}\Exp[\,\MST\mid \calF\A{i}] \Prob[\calF\A{i}]
\leq  \sum_{i=1}^{n-1}\bigl(\frac{\epsilon}{2}\bigr)^i  \Exp[\,\MST\mid \calF\langle 1\rangle] \Prob[\calF\A{1}]
\leq  \epsilon\Exp[\,\MST\mid \calF\langle 1\rangle] \Prob[\calF\A{1}].
$
Now, we prove the claim.
First, we rewrite the LHS and the RHS as follows:
$$
\Exp[\,\MST\mid \calF\A{i+1}]\cdot \Prob[\calF\A{i+1}]
=\sum_{|S|=i+1} \sum_{F_S\in \calF_S} \sum_{H_{\bS}\in \calH_{\bS}}
\bigl(\,
\Prob[(F_S,H_{\bS})]\cdot
\MST(F_S, H_{\bS})\,\bigr),
$$
$$
\Exp[\,\MST\mid \calF\A{i}]\cdot \Prob[\calF\A{i}]
=\sum_{|S'|=i} \sum_{F'_{S'}\in\calF_{S'}} \sum_{H'_{\bS'}\in \calH_{\bS'}}
\bigl(\,
\Prob[(F_S,H_{\bS})]\cdot
\MST(F'_{S'}, R_{\bar{S}'})\,\bigr).
$$
For each pair $(F_S, H_{\bS})$,
let $C(F_S, H_{\bS})=
\Prob[F_S, H_{\bS}]\cdot \MST(F_S, H_{\bS})$.
%For each pair $(F', R_{\bar{S}'})$ with $|S|=i$,
%we define $B(F', R_{\bar{S}'})$ in a similar way.
Think each pair $(F_S, H_{\bS})$ with $|S|=i+1$ as a seller
and each pair $(F'_{S'}, H'_{\bS'})$ with $|S'|=i$ as a buyer.
The seller $(F_S, H_{\bS})$ want to sell the term $C(F_S, H_{\bS})$
and the buyers want to buy all these terms.
The buyer $(F'_{S'}, H'_{\bS'})$ has a budget of $C(F'_{S'}, H'_{\bS'})$.
We show there is a charging scheme such that
every term $C(F_S, H_{\bS})$ is fully paid by the buyers and
each buyer spends at most an $\frac{\e}{2}$ fraction of her budget.
Note that the existence of such a charging scheme suffices to prove the lemma.

Suppose we are selling the term $C(F_S, H_{\bS'})$.
Consider the following charging scheme.
Suppose $v\in S$ is the node closest to any node in $\bS$.
Let $S'=S\setminus v$ and $F'_{\S'}$ be the restriction of $F_S$ to all
coordinates in $S$ except $v$.
We say $(F'_{S'}, H'_{\bS'})$ is consistent with  $(F_S, H_{\bS})$,
denoted as $(F'_{S'}, H'_{\bS'})\consistent (F_S, H_{\bS})$,
if $H_{\bS}$ agrees with  $H'_{\bS'}$ for all vertices in $\bS$,
and $F_S$ agrees with  $F'_{S'}$ for all vertices in $S'$.
Intuitively, $(F'_{S'}, H'_{\bS'})$ can be obtained from $(F_S,H_{\bS})$
by sending $v$ to an arbitrary point in $\H$.
Let $$
Z(F_S, H_{\bS})=
\sum_{(F'_{S'}, H'_{\bS'})\consistent (F_S, H_{\bS})} \Prob[(F'_{S'}, H'_{\bS'})].
$$
For each buyer $(F'_{S'},H'_{\bS'})\sim (F_S, H_{\bS})$,
we charge her the following amount of money
$$
\frac{\Prob[(F'_{S'},H'_{\bS'})]}
{Z(F_S, H_{\bS})}
C(F_S, H_{\bS})
$$
It is easy to see that $C(F_S, H_{\bS})$ is fully paid by all buyers
consistent with $(F_S, H_{\bS})$.
It remains to show that each buyer $(F'_{S'}, H'_{\bS'})$
has been charged at most $\frac{\epsilon}{2}C(F'_{S'}, H'_{\bS'})$.
By the above charging scheme,
the terms in LHS that are charged to buyer $(F'_{S'}, H'_{\bS'})$
are consistent with $(F'_{S'}, H'_{\bS'})$.
Therefore, the total amount charged to buyer $(F'_{S'}, H'_{\bS'})$ is
\begin{align*}
\sum_{(F_S, H_{\bS})\consistent (F'_{S'}, H'_{\bS'})}
\frac{\Prob[F'_{S'},H'_{\bS'}]}
{Z(F_S, H_{\bS})}
C(F_S, H_{\bS})
&\leq
4\MST(F'_{S'}, H'_{\bS'}) \cdot \sum_{(F_S, H_{\bS})\consistent (F'_{S'}, H'_{\bS'})}
\frac{\Prob[F'_{S'},  H'_{\bS'}]}
{Z(F_S, H_{\bS})}
\Prob[(F_S, H_{\bS})]\\
=&\, 4\MST(F'_{S'}, H'_{\bS'}) \Prob[F'_{S'},H'_{\bS'}]\cdot
\sum_{(F_S, H_{\bS})\consistent (F'_{S'}, H'_{\bS'})}
\frac{\Prob[F_S, H_{\bS}]}
{Z(F_S, H_{\bS})}\\
\leq &\, 4\MST(F'_{S'}, H'_{\bS'}) \Prob[F'_{S'},H'_{\bS'}]\cdot
\sum_{v\in \bS'} \frac{\Prob(v\in \calF)}{\Prob(v\in \H)} \\
\leq &\, \frac{\epsilon}{2}\MST(F'_{S'}, H'_{\bS'}) \Prob[F'_{S'}, H'_{\bS'}]
\end{align*}
The first inequality follows from Lemma~\ref{lm:mstchange}.
To see the second inequality,
for a fixed vertex $v$, consider the quantity
$
\sum_{(F_S, H_{\bS})\consistent (F'_{S'}, H'_{\bS'}), \bS=\bS'\setminus \{v\}}
\frac{\Prob[F_S, H_{\bS}]}{Z(F_S, H_{\bS})}.
$
By the definition of $Z$, we can see that the denominators of all terms are in fact the same.
Canceling out the same multiplicative terms from the numerators and the denominator,
we can see it is at most $\frac{\Prob(v\in \calF)}{\Prob(v\in \H)}$.
\qed
%\end{proof}
\end{proof}

\section{Proof of Lemma \ref{lm:samTj}}

\begin{proof}
W.l.o.g, we assume that the points in $T$ are $s_1,\ldots, s_{|T|}$. We denote the event that among points in $\{s_i\}_{1\leq i\leq a}$ there are exactly $b$ points are present by $E[T,a,b]$ and denote the probability of $E[T,a,b]$ by $\Prob[T,a,b]$. Note that our goal is to give a sampler conditioning on the event $E[|T|,j]$. Since we have the following two properties, we can compute $\Prob[T,|T|,j]$ in polynomial time first.

\begin{enumerate}
\item If $a < b$, $\Prob[T,a,b]=0$. If $a=b$, $\Prob[T,a,b]=\prod_{1\leq l\leq a}p_l$. If $b=0$, $\Prob[a,b]=\prod_{1\leq l\leq a}(1-p_l)$.
\item For $a>b$ and $b\geq 1$, $\Prob[a,b]=p_a \Prob[a-1,b-1]+(1-p_a) \Prob[a-1,b]$.
\end{enumerate}

Then we use this dynamic programming to show how to sample. Consider point $s_{|T|}$ firstly. We sample it present with probability $p_{|T|} \Prob[T,|T|-1,j-1]/\Prob[T,|T|,j]$ and then sample conditioning on the event $E[T,|T|-1,j-1]$. Otherwise, we do not sample it with probability $(1-p_{|T|}) \Prob[T,|T|-1,j]/\Prob[T,|T|,j]$ and then sample conditioning on the event $E[T,|T|-1,j]$. We do this process recursively until $j$ points are sampled.
\qed
\end{proof}

\section{Proof of Lemma \ref{lm:samMST_k}}

\begin{proof}
Note that $\Prob[L_i]=\Prob[T^*_{i,1}\A{1}]\cdot \Prob[T^*_{i,2}\A{1}]\cdot \Prob[\calT_i\A{k,\geq 1}]$. Since we can compute $\Prob[T^*_{i,1}\A{1}]$ and $\Prob[T^*_{i,2}\A{1}]$ in polynomial time, the problematic part is how to compute $\Prob[\calT_i\A{k,\geq 1}]$. Note that each two components $T_1,T_2$ in $\calT_i$ have no common point. So $T_1\A{\geq 1}$ and $T_2\A{\geq 1}$ are independent. Note that for each component $T_j$, we can compute $q_j=T_j\A{\geq 1}$ in polynomial time. We use a dynamic program to compute $\Prob[\calT_i\A{k,\geq 1}]$. Without loss of generality, assume $\calT_i=\{T_{i,j} \}_{1\leq j\leq m-i}$. We denote the event that in $\{T_{i,j} \}_{1\leq j\leq a}$ there are exactly $b$ components containing no less than 1 point by $E[a,b]$ ($1\leq a\leq m-i$, $0\leq b\leq k$) and denote the probability of $E[a,b]$ by $\Prob[a,b]$. Note that our goal is to compute $E(m-i,k)$ in polynomial time. Since we have the following two properties, we can compute $\Prob[m-i,k]$ in polynomial time.

\begin{enumerate}
\item If $a < b$, $\Prob[a,b]=0$. If $a=b$, $\Prob[a,b]=\prod_{1\leq j\leq a}q_j$. If $b=0$, $\Prob[a,b]=\prod_{1\leq j\leq a}(1-q_j)$.
\item For $a>b$ and $b\geq 1$, $\Prob[a,b]=q_a \Prob[a-1,b-1]+(1-q_a) \Prob[a-1,b]$.
\end{enumerate}

Then we show how to sample conditioning on $L_i$. Since we have Lemma~\ref{lm:samTj}, we only need to show how to sample $k$ components in $\calT_i$ which have no less than 1 point present conditioning on $E[m-i,k]$. In fact, the dynamic program is very helpful. Consider component $T_{i,m-i}$. We sample this component with probability $q_{m-i} \Prob[m-i-1,k-1]/\Prob[m-i,k]$ and then sample conditioning on $E[m-i-1,k-1]$. On the other hand, we do not sample this component with probability $(1-q_{m-i}) \Prob[m-i-1,k]/\Prob[m-i,k]$ and then sample conditioning on $E[m-i-1,k]$. We do this process recursively until $k$ components are sampled.
\qed
\end{proof}

\section{Proof of Lemma \ref{lm:samCP_k}}
\begin{proof}
We denote the event that in $\{T_{i,j} \}_{1\leq j\leq a}$ there are exactly $b<k$ collisions by $E[a,b]$ ($1\leq a\leq m-i$, $0\leq b\leq k$) and denote the probability of $E[a,b]$ by $\Prob[a,b]$. Let the total points in $T_{i,j}$ be $n_{i,j}$. We give the following dynamic programming.

\begin{enumerate}
\item If $\sum_{1\leq j\leq a}{n_{i,j}\choose 2} < b$, $\Prob[a,b]=0$. If $b\leq 0$, $\Prob[a,b]=\prod_{1\leq j\leq a}\Prob[T_{i,j}\A{0}]$.
\item For $\sum_{1\leq j\leq a}{n_{i,j}\choose 2} > b$ and $1\leq b\leq k-1$, $\Prob[a,b]=\sum_{0\leq l\leq n_{i,a}} \Prob[T_{i,a}\A{l}]\cdot E[a-1,b-{l\choose 2}]$.
\end{enumerate}

By Lemma~\ref{lm:samTj}, in a component $T$, there exists a polynomial algorithm for computing $\Prob[T\A{\geq l}$ for $0\leq l\leq |T|$ and a polynomial uniform sampler to sample points conditioning on $T\A{\geq j}$.
Above all, we can compute $\Prob[m-i-1,l]$ for $1\leq l\leq k-1$ in polynomial time.
Then we could rewrite $\Prob[L_i]$ as follows:
$$
\Prob[L_i]=\sum_{1\leq a\leq |T^*_{i,1}|, 1\leq b\leq |T^*_{i,2}|} \Prob[T^*_{i,1}\A{a}]\cdot \Prob[T^*_{i,2}\A{b}]\cdot \sum_{k-{a\choose 2}-{b\choose 2}-ab\leq l\leq k-1-{a\choose 2}-{b\choose 2}} \Prob[m-i-1,l]
$$
Note that we could compute $\Prob[L_i]$ in polynomial time by the above equality. Moreover, this format of $\Prob[L_i]$ could help us obtain a polynomial uniform sampler conditioning on $L_i$. Now we describe our sample steps. We sample the event $T^*_{i,1}\A{a}\wedge T^*_{i,2}\A{b}$ at first. Then conditioning on $k-{a\choose 2}-{b\choose 2}-ab\leq l\leq k-1-{a\choose 2}-{b\choose 2}$, we sample the event $E[m-i-1,l]$. Similarly, we use the dynamic programming to sample the number of points present in each component in $\calT_i$. Finally, by lemma~\ref{lm:samTj}, we could sample each point present or not in polynomial time.
\qed
\end{proof}

\section{Proof of Lemma~\ref{lm:lm2core}}

\begin{proof}
Suppose $s =\arg\max_{s'} \{p_{vs'}\mid s' \in \H_1\}$,
and $t =\arg\max_{t'}\{p_{vt'}\mid t' \in \H_2\}$.
Obviously, we have $p_{vs} \geq \frac{p_v(\H_1)}{m}$ and $p_{vt} \geq \frac{p_v(\H_2)}{m}$.
So it suffices to show $\Exp[\MM]\geq \min\{p_{vs},p_{vt}\}\cdot \dist(s,t)$.
We first see that
\begin{align*}
\Exp[\MM]&\geq p_{vs} \Exp[\MM\mid v \realize s]+ p_{vt} \Exp[\MM\mid v \realize t] \\
&\geq \min\{p_{vs},p_{vt}\} \Bigl(\Exp[\MM\mid v \realize s]
+\Exp[\MM\mid v \realize t]\Bigr).
\end{align*}
Then it is sufficient to prove that $\Exp[\MM\mid v \realize s]+\Exp[\MM\mid v \realize t]\geq \dist(s,t)$.
Fix a realization of all nodes except $v$ and condition on this event.
Consider the two minimum perfect matchings, one for the case $v \realize s$, (denoted as $\MM_1$) and
the other one for $v \realize t$ (denoted as $\MM_2$).
Consider the symmetric difference
$$\MM_1\oplus \MM_2.$$
We can see that it is a path $(s, p_1, p_2, \ldots,p_k ,t)$, such that $(s,p_1)\in \MM_1$,$(p_1,p_2)\in \MM_2,\ldots,$ $(p_k,t)\in \MM_2$.
So $\MM_1+\MM_2 \geq  \dist(s,t)$ by the triangle inequality.
Therefore, we have $\Exp[\MM\mid v \realize s]+\Exp[\MM\mid v \realize t]\geq \dist(s,t)$.
\qed
\end{proof}

\linesnotnumbered
\begin{algorithm}
\caption{Estimating the first two terms for $\MM$}\label{alg:estMM}
\nl \textbf{Input:} The node set $\V$, the point set $\P$, and the \core\ $\H_1,\ldots, \H_k$.\\
\textbf{-- Procedure 1: Estimating $\Exp[\,\MM\mid \calF\A{0} \,] \cdot \Prob[ \calF\A{0}]$}\\
\nl Take $N_1=O(\frac{n^2m^5}{\e^4}\ln n)$ independent samples. Set $A\leftarrow \emptyset$ at the beginning.\\
\nl For each sample $G_i$, if it satisfies $\H\A{n}$, $A\leftarrow A\cup \{G_i\}$.\\
$T_0\leftarrow \frac{1}{N_1}\sum_{G_i\in A}\MM(G_i)$.\\
\textbf{-- Procedure 2: Estimating $\Exp[\,\MM\mid \calF\A{1} \,] \cdot \Prob[ \calF\A{1}]$}\\
\nl For each node $v$, set $B_v\leftarrow \{s\mid s\in \calF, \dist(s,\H(v))<\frac{4nD}{\e }$. Let $\Cl(v)$ be the event that $v$ is the only node that realizes to some node $s\notin \H(v)$ and $s\in B_v$.\\
\nl Conditioning on $\Cl(v)$, take $N_1=O\bigl( \frac{n^2m^5}{\e^{5}}\ln n\bigr)$ independent samples.
Let $A_v\leftarrow \{G_{v,i}\mid 1\leq i\leq N_2\}$ be the set of $N_1$ samples for $\Cl(v)$.\\
\nl $T_v\leftarrow \frac{1}{N_1}\sum_{G_{v,i}\in A_v}\MM(G_{v,i})$  ~~~(estimating $\Exp[\,\MM\mid \Cl(v)]$)\\
\nl $T_1\leftarrow \sum_{v\in \V}\Bigl(\Prob[\Cl(v)]T_v+\sum_{s\in \calF\setminus B_v}\Prob[\calF\A{v}\wedge v\realize s]\,\dist(s,\H(v))\,\Bigr)$.\\
\nl \textbf{Output:} $T_0+T_1$
\end{algorithm}



We need the following structural result about minimum perfect matchings,
which is essential for our charging argument.

Suppose $S$ is the set of nodes that are out of their homes.
We use $\calF_S$ and $\calH_{\bS}$
to denote the set of all realizations of the all nodes in $S$ to points in $\calF$,
and the set of realizations of $\bS=V\setminus S$ to points in $\H$ respectively.
We use $\MM(F_S, H_{\bS})$ to denote the length of the minimum perfect matching
under the realization $(F_S, H_{\bS})$, where $F_S\in \calF_S$ and $H_{\bS}\in \calH_{\bS}$.
The following combinatorial fact plays the same role
in the charging argument as Lemma~\ref{lm:mstchange} does in the previous section.
Different from the MST problem,
we can not achieve a similar bound to the one in Lemma~\ref{lm:mstchange} since
$\MM(F_S, H_{\bS})$ may decrease significantly if we only sending only one node outside home back to its home.
However, we show that in such case, if we send one more node back home,
$\MM(F_S, H_{\bS})$ can still be bounded.

\begin{lemma}
\label{lm:del1or2}
%A pair $(F_S,H_{\bS})$ means for each node $s\in S$,
%$s$ locates on a certain point out of $\textcircled{s}$, and for each node $s\in \bar{s}$, $s\realize \textcircled{s}$.
Fix a realization $(F_S,H_{\bS})$.
We use  $\ell(v)$ to denote $\dist(v, \Home(v))$ for all nodes $v\in S$.
Suppose $v_1\in S$ has the smallest $\ell$ value and $v_2$ has the second smallest $\ell$ value.
Let $S'=S\setminus \{v_1\}$, $S''=S'\setminus \{v_2\}$.
Further let $(F_{S'}, H_{\bS'})$ be a realization obtained from $(F_S, H_{\bS})$ by sending $v_1$ to
a point in its home $\Home(v_1)$
and
$(F_{S''}, H_{\bS''})$ be a realization obtained from $(F_{S'}, H_{\bS'})$ by sending $v_2$ to
a point in its home $\Home(v_2)$.
Then we have that
$
\MM(F_S,H_{\bS})\leq 2(m+2)\MM(F_{S'},H_{\bS'})+2(m+2)\MM(F_{S''},H_{\bS''})
$
\end{lemma}

What remains is to establish the following key lemma. The proof is
similar to, but more involved than that of Lemma~\ref{lm:mstcharge}.
\begin{lemma}
\label{lm:matchingcharge}
For any $\epsilon>0$,
if $H$ satisfies the properties in Lemma~\ref{lm:matchinghome}, we have that
$$
\sum_{i> 1}\Exp[\MM\mid \calF\A{i}]\cdot \Prob[\calF\A{i}]\leq \epsilon\cdot \Exp[\MM\mid \calF\A{0}] \cdot \Prob[\calF\A{0}]+\epsilon\cdot \Exp[\MM\mid \calF\langle 1\rangle]\cdot \Prob[\calF\A{1}].
$$
\end{lemma}


\section{Proof of Lemma \ref{lm:est0MM}}

\begin{proof}
Note that $\Prob[\H\A{n}]$ is close to $1$ (by union bound) and can be computed exactly.
To estimate $\Exp[\MM\mid \H\A{n}]]$, the algorithm takes the average of $N_1=O(\frac{n^2m^5}{\e^4}\ln n)$ samples. Note that conditioned on $\H\A{n}$, the minimum perfect matching could be at most $nD$.
We distinguish the following two cases.
\begin{enumerate}
\item
$\Exp[\MM\mid \H\A{n}]\geq \frac{\e}{2}\Exp[\MM]\geq\Omega(\frac{\e^2 D}{nm^5})$. We could get a $(1\pm \epsilon)$-approximation using the Monte Carlo method with $O(\frac{n^2m^5}{\e^4}\ln n)$ samples. This is because the maximum possible $\MM$ length is at most $nD$ and therefore we have poly-bounded.
\item
$\Exp[\MM\mid \H\A{n}]< \frac{\e }{2}\Exp[\MM]$. Then the probability that the sample average is larger than $\epsilon \Exp[\MM]$ is at most $\poly(\frac{1}{n})$ by Chernoff Bound.
We can thus ignore this part safely. \qed
\end{enumerate}
\end{proof}

\section{Proof of Lemma \ref{lm:est1MM}}

\begin{proof}
To compute the second term, we first rewrite it as follows:
$$\Exp[\MM\mid \calF\A{1} ]\cdot \Prob[\H\A{1}]
=\sum_{v\in \V} \Bigl(\,\sum_{s\notin \Home(v)} \Prob[\calF\A{v}\wedge v\realize s]\
\Exp[\MM\mid \calF\A{v}, v\realize s ]\,\Bigr).
$$
%We can easily see that $\Prob[F\A{v}\wedge v\realize s]$ can be computed precisely in poly-time.
Fix a particular node $v$.
To estimate $\sum_{s\in \calF} \Prob[\calF\A{v}\wedge v\realize s]\, \Exp[\MM\mid \calF\A{v}, v\realize s ]$, we consider the following two situations:
\begin{enumerate}
\item
Point $s\in B^v$, i,e, $\dist(s,\H(v))<\frac{4nD}{\e }$.

We estimate the sum for all $s\in B^v$. Notice that the sum is
in fact $\Prob[\Cl(v)]\cdot\E[\,\MM\mid \Cl(v) ]$.
%Here $v\realize \Cl(s)$ means that node $v$ is present at some point $s\in \Cl(s)$.
We can see that $\Prob[\Cl(v)]$ can be computed exactly in linear time.
We argue the quality of the estimation taken on $N_2=O\bigl( \frac{n^2m^5}{\e^{5}}\ln n\bigr)$ samples is good
by considering the following two cases:
%If
%$$\sum_{s:\dist(u,H)<n^{10}}\Exp[\,\MST \mid F\A{v}, v\realize s ]\cdot\Prob[v\realize s \mid F\A{v}]
%\geq \frac{1}{n^3}\Exp[\,\MST \mid H\A{n}]]\geq \frac{1}{(mn)^5}\diam(H),
%$$
    \begin{enumerate}
    \item Assume that $
    \E[\,\MM\mid \Cl(v) ]
    \geq \frac{1}{2}\Exp[\,\MM \mid \H\A{n}]\geq \Omega\Bigl(\frac{\e D}{nm^5}\Bigr).
    $
    In this case, we have poly-bounded.
    This is because under the condition $\Cl(v)$,
    the maximum possible length of any minimum spanning tree is $O(\frac{nD}{\e})$.
    Hence we can use Monte Carlo to get a $(1\pm \epsilon)$-approximation
    of $\E[\,\MM\mid \Cl(v) ]$ with $O\bigl( \frac{nm^2}{\e^{5}}\ln n\bigr)$ samples.
    \item Otherwise, we assume that

    $
    \E[\,\MM\mid \Cl(v) ]
    \leq \frac{1}{2}\Exp[\,\MM \mid \H\A{n}]].
    $
    The probability that the sample average is larger than $\Exp[\MM\mid \H\A{n}]] $
    is at most $\poly(\frac{1}{n})$ by Chernoff Bound. The probability that for all nodes $v$, the sample average are
    at most $\Exp[\MM\mid \H\A{n}]]$ is at least $1-\poly(\frac{1}{n})$ by union bound.
    If this is the case, we can see their total contribution
    to the final estimation of $\E[\MM]$ is less than $\e \Exp[\,\MM \mid \H\A{n}]] \Prob[\H\A{n}] $.
    In fact, this is because
    \begin{align*}
    & \sum_{v\in V} \Prob[\Cl(v)]\cdot\E[\,\MM\mid \Cl(v) ]\leq \sum_{v\in V}\Prob[\Cl(v)]\cdot \Exp[\,\MM \mid \H\A{n}]] \\
    & <\e \Exp[\,\MM \mid \H\A{n}]] \Prob[\H\A{n}].
    \end{align*}
    The second inequality is due to the fact that $\sum_{v\in V}\Prob[\Cl(v)]\leq n-\sum_{v\in V} p_v(\H(v))\leq \frac{\e}{m^3}<\e \Prob[\H\A{n}]$.
    \end{enumerate}
\item
Point $s\in F\setminus B^v$, each term has $\dist(s,\H(v))>\frac{4nD}{\e }$.
The algorithm uses $\dist(s,\H(v))$
as the estimation of $\Exp[\MM\mid \calF\A{v}, v\realize s ]$.
Note that the length of $\MM$ is always at least $\dist(s,\H(v))-nD\geq (1-\frac{\e}{4})\dist(s,\H(v))$. This is because such an instance $\MM$ contains a path from $s$ to some point $t\in \H(v)$ deleting no more than $n$ segments of length at most $D$ (each segment is in some $\H_j$).
On the other hand, at most $\dist(s,\H(v))+nD \leq (1+\frac{\e}{4}) \dist(s,\H(v))$. So it is a $(1\pm\epsilon)$-estimation.
\qed
\end{enumerate}

\eat{
\begin{enumerate}
\item
$d(p,\textcircled{s})< n^{10}D$.
Fix a particular node $s$.
We estimate the sum $\sum_{p:d(p,\textcircled{s})<n^{10}}\Exp[\MM \mid F\A{\{s\}}, s\realize p ]\cdot\Prob[F\A{\{s\}}\wedge s\realize p]$
by taking the average of $xxx$ independent samples.
If
$$\sum_{p:d(p,H)<n^{10}}D\Exp[\MM \mid F\A{\{s\}}, s\realize p ]\cdot\Prob[F\A{\{s\}}\wedge s\realize p]
\geq \frac{1}{n^3}\Exp[\MM]\geq \frac{D}{(mn)^8},
$$
by Lemma~\ref{}, our estimate is a $(1\pm \epsilon)$-approximation with high probability.
Otherwise, we have that
$$
\Exp[\MM\mid F\A{1} ]\cdot \Prob[H\A{1}]\leq \frac{1}{n^3} \Exp[\MM]
$$
Therefore,
the probability that the sample average is larger than $\epsilon \Exp[\MM]$
is at most $\frac{1}{n^2}$ by Markov's inequality.
Similarly, a sample average that is much smaller than its expectation causes no problem neither since
the expectation contributes less than $\frac{1}{n^3}$ fraction of the final solution by our assumption,
thus can be ignored safely.\\
\end{enumerate}
}
\end{proof}

\section{Proof of Lemma \ref{lm:del1or2}}

\begin{proof}
Let $\d=\min_v \ell(v)$ and $D=\max_i \diam(H_i)$. Note that $d\geq \frac{D}{m}$ as $d\geq 2T$ and $D\leq 2mT$.
We distinguish the following three cases:
\begin{enumerate}
\item
$\MM(F_S,H_{\bS})\leq \frac{\d}{2}$.
Using a similar argument to the one in Lemma~\ref{lm:lm2core}, we have
$$
\MM(F_{S'},H_{\bS'})+\MM(F_S,H_{\bS})\geq \ell(v)=\d
$$
So, we have  $\MM(F_S,H_{\bS})\leq \MM(F_{S'},H_{\bS'})$ in this case.
\item
$\MM(F_S,H_{\bS})\geq (m+2)\d$.
%Let $s_1$ locate on a point in its corresponding ball. We can get a matching for $(F_{S^{'}},H_{\bar{S^{'}}})$.
By the triangle inequality,  we can see that
$$
\MM(F_{S'},H_{\bS'})+(m+1)d\geq \MM(F_{S'},H_{\bS'})+d+D\geq \MM(F_S,H_{\bS})
$$
So, we have $\MM(F_S,H_{\bS})\leq (m+2)\MM(F_{S'},H_{\bS'})$.
\item
$\frac{\d}{2}\leq \MM(F_S,H_{\bS})\leq (m+2)\d$.
\begin{enumerate}
\item
$\MM(F_{S'},H_{\bS'})\geq \frac{\d}{2}$.
We directly have $\MM(F_S,H_{\bS})\leq 2(m+2)\MM(F_{S'},H_{\bS'})$.
\item
$\MM(F_{S'},H_{\bS'})\leq \frac{\d}{2}$.
By Lemma~\ref{lm:lm2core}, we have
$$
\MM(F_{S'},H_{\bS'})+\MM(F_{S''},H_{\bS''})\geq \d
$$
Then we have $\MM(F_S,H_{\bS})\leq 2(m+2)\MM(F_{S''},H_{\bS''})$.
\end{enumerate}
\end{enumerate}
So we prove the lemma. \qed
\end{proof}

\section{Proof of Lemma \ref{lm:matchingcharge}}

\begin{proof}
We claim that for any $i > 1$,
$$
\Exp[\MM\mid \calF\A{i+1}]\cdot \Prob[\calF\A{i+1}]\leq
\frac{\epsilon}{6}\bigl(\,\Exp[\MM\mid \calF\A{i}]\cdot \Prob[\calF\A{i}]+\Exp[\MM\mid \calF\A{i-1}]\cdot \Prob[\calF\A{i-1}]\,\bigr)
$$
If the claim is true, the lemma can be proven easily as follows.
For ease of notation, we use $A(i)$ to denote $\Exp[\MM\mid \calF\A{i}]\cdot \Prob[\calF\A{i}]$.
First, we can see that
\begin{align*}
A(i+2)+A(i+1) \leq \frac{\epsilon}{6} A(i+1) +\frac{2\epsilon}{6}A(i) +\frac{\epsilon}{6} A(i-1)\leq \frac{\epsilon}{2}(A(i)+A(i-1)).
\end{align*}
So if $i$ is odd,
$A(i+2)+A(i+1) \leq (\frac{\epsilon}{2})^{(i+1)/2}(A(1)+A(0)).$
Therefore, $\sum_{i>1} A(i)\leq \frac{\epsilon/2}{1-\epsilon/2} (A(1)+A(0))\leq \e(A(1)+A(0))$.
%\begin{align*}
%& \leq \Bigl(\frac{3\epsilon}{n^2}\Bigr) \bigl(\,\Exp[\MM\mid F\A{i}]\cdot \Prob[F\A{i}]+\Exp[\MM\mid F\A{i-1}]\cdot \Prob[F\A{i-1}]\,\bigr)
%\end{align*}
%could use induction to prove an even stronger result.
%$$
%\sum_{i> 1}\Exp[\MM\mid F\A{i}]\cdot \Prob[F\A{i}]\leq (1-\frac{1}{n})\epsilon
%\cdot (\Exp[\MM\mid F\A{0}] \cdot \Prob[F\A{0}]+ \Exp[\MM\mid F\langle 1\rangle]\cdot \Prob[F\A{1}])
%$$
%The basic step: $n=2$, it's obvious. $n=3$, we have
%\begin{align*}
%&\Exp[\MM\mid F\A{3}]\cdot \Prob[F\A{3}]+\Exp[\MM\mid F\A{4}]\cdot \Prob[F\A{4}]\\
%\leq &(\frac{\epsilon}{4^2}+(\frac{\epsilon}{4^2})^2)\cdot(\Exp[\MM\mid F\A{0}] \cdot \Prob[F\A{0}]+(\frac{2\epsilon}{4^2}+(\frac{\epsilon}{4^2})^2)\cdot\Exp[\MM\mid F\langle 1\rangle]\cdot \Prob[F\A{1}]\\
%\leq &(1-\frac{1}{4})\epsilon \cdot (\Exp[\MM\mid F\A{0}] \cdot \Prob[F\A{0}]+ \Exp[\MM\mid F\langle 1\rangle]\cdot \Prob[F\A{1}])
%\end{align*}
%The induction step: If $n-1\geq 4$ is satisfied, then consider $n$ nodes.
%\begin{align*}
%\sum_{i=2}^{n}\Exp[\MM\mid F\A{i}]\cdot \Prob[F\A{i}]\leq
%& \Exp[\MM\mid F\A{0}]\cdot \Prob[F\A{0}]+ \sum_{i=1}^{n-2}\Exp[\MM\mid F\A{0}]\cdot \Prob[F\A{0}]
%\sum_{i=2}^{n-1}\Exp[\MM\mid F\A{i}]\cdot \Prob[F\A{i}]+\Exp[\MM\mid F\A{n}]\cdot \Prob[F\A{n}]\\
%\leq & \sum_{i=2}^{n-1}\Exp[\MM\mid F\A{i}]\cdot \Prob[F\A{i}]+\frac{\epsilon}{n^2}\bigl(\,\Exp[\MM\mid F\A{n}]\cdot \Prob[F\A{n}]+\Exp[\MM\mid F\A{n-1}]\cdot \Prob[F\A{n-1}]\,\bigr)\\
%\leq & \sum_{i=2}^{n-1}\Exp[\MM\mid F\A{i}]\cdot \Prob[F\A{i}]+ \frac{\epsilon}{n^2} \cdot \sum_{i=2}^{n-1}\Exp[\MM\mid F\A{i}]\cdot \Prob[F\A{i}]\\
%\leq & (1+\frac{\epsilon}{n^2})(1-\frac{1}{n-1})\epsilon \cdot (\Exp[\MM\mid F\A{0}] \cdot \Prob[F\A{0}]+ \Exp[\MM\mid F\langle 1\rangle]\cdot \Prob[F\A{1}])~(induction)\\
%\leq & (1-\frac{1}{n})\epsilon \cdot (\Exp[\MM\mid F\A{0}] \cdot \Prob[F\A{0}]+ \Exp[\MM\mid F\langle 1\rangle]\cdot \Prob[F\A{1}])
%\end{align*}
Now, we prove the claim. Again, we rewrite the LHS as
$$
\Exp[\MM\mid \calF\A{i+1}]\cdot \Prob[\calF\A{i+1}]
=\sum_{|S|=i+1} \sum_{F_S} \sum_{H_{\bS}}
\Bigl(\,
\Prob[ F_S,  H_{\bS}]\cdot
\MM(F_S, H_{\bS})\,\Bigr).
$$
%Here $ H_{\bS}$ means for each $s\in \bS, s\realize \textcircled{s}$. \\
Similarly, we have the RHS to be
$$
\Exp[\MM\mid \calF\A{i}]\cdot \Prob[\calF\A{i}]
=\sum_{|S'|=i} \sum_{F_{S'}} \sum_{H_{\bS'}}
\Bigl(\,
\Prob[ F_{S'},  H_{\bS'}]\cdot
\MM(F_{S'}, H_{\bS'})\,\Bigr)
$$
$$
\Exp[\MM\mid \calF\A{i-1}]\cdot \Prob[\calF\A{i-1}]
=\sum_{|S^{''}|=i-1} \sum_{F_{S^{''}}} \sum_{H_{\bS''}}
\Bigl(\,
\Prob[F_{S^{''}},  H_{\bar{S^{''}}}]\cdot
\MM(F_{S^{''}}, H_{\bar{S^{''}}})\,\Bigr)
$$
Let $C(F_S, H_{\bS})=
\Prob[ F_S,  H_{\bS}]\cdot \MM(F_S, H_{\bS})$.
Think all $(F_{S'},H_{\bS'})$ with $|S^{'}|=i$
and all $(F_{S''},H_{\bS''})$ with $|S^{''}|=i-1$
as buyers.
The buyers want to buy all terms in LHS.
The budget of buyer $(F_{S'},H_{\bS'})$ is $C(F_{S'},H_{\bS'})$.
We show there is a charging scheme such that
every term $C(F_{S}, H_{\bS})$ is fully paid by the buyers and
each buyer spends at most an $\frac{\e}{6}$ fraction of her budget.

Suppose we are selling the term $C(F_S, H_{\bS})$.
Consider the following charging scheme.
Suppose $v\in S$ the node that realizes to point $f\in F_S$
which is the closest point to $H_{\bS}$ in $F_S$.
Suppose $t\in S$ the node that is realized to point $F_t\in F_S$
which is the second closest point to $H_{\bS}$ in $F_S$.
Let $S'=S\setminus \{v_1\}$, $S''=S'\setminus \{v_2\}$.
If $(F_{S'}, R_{\bS'})$ is obtained from $(F_S, H_{\bS})$ by sending $v_1$ to
a point in its home $\Home(v_1)$,
we say $(F_{S'}, R_{\bS'})$
is consistent with  $(F_{S}, R_{\bS})$,
denoted as $(F_{S'}, R_{\bS'})\consistent (F_{S}, R_{\bS})$.
If $(F_{S''}, R_{\bS''})$ is obtained from $(F_{S'}, H_{\bS'})$ by sending $v_2$ to
a point in its home $\Home(v_2)$,
we say $(F_{S''}, R_{\bS''})$
is consistent with  $(F_{S'}, R_{\bS'})$,
denoted as $(F_{S'}, R_{\bS'})\consistent (F_{S}, R_{\bS})$.
Let
$$
Z(F_{S}, H_{\bS})=
\sum_{(F_{S'}, H_{\bS'})\consistent (F_{S}, H_{\bS})} \Prob[(F_{S'}, H_{\bS'})],
\quad\text { and }$$
$$
Z(F_{S'}, H_{\bS'})=
\sum_{(F_{S''}, H_{\bS''})\consistent (F_{S'}, H_{\bS'})} \Prob[F_{S''}, H_{\bS''}]
$$
For each buyer $(F_{S'},H_{\bS'})\sim (F_{S}, H_{\bS})$,
we charge $(F_{S'}, H_{\bS'})$ the following amount of dollars
$$
\frac{\Prob[F_{S'},  H_{\bS'}]}
{Z(F_{S}, H_{\bS})}
\Prob[ F_S,  H_{\bS}]\cdot 2(m+2)\MM(F_{S'}, H_{\bS'})
$$
and we charge every buyer $(F_{S''}, H_{\bS''})$ consistent with $(F_{S'}, H_{\bS'})$ the following amount of money
\begin{align*}
%&\frac{\Prob[F_{S'}, H_{\bS'}]}
%{Z(F_{S}, H_{\bS})}\cdot \frac{\Prob[F_{S''},  H_{\bS''}]}
%{Z(F_{S'}, H_{\bS'})}
%\Prob[ F_S,  H_{\bS}]\cdot 2(n+2)\MM(F_{S''}, H_{\bS''})\\
\frac{\Prob[F_{S}, H_{\bS}]}
{Z(F_{S}, H_{\bS})}\cdot \frac{\Prob[F_{S'},  H_{\bS'}]}
{Z(F_{S'}, H_{\bS'})}
\Prob[ F_S'',  H_{\bS''}]\cdot 2(m+2)\MM(F_{S''}, H_{\bS''})
\end{align*}
In this case, we say $(F_{S''}, H_{\bS''})$ is a {\em sub-buyer} of the term $C(F_S, H_{\bS})$.
By Lemma~\ref{lm:del1or2}, we can see that $A(F_S, H_{\bS})$ is fully paid.
To prove the claim,
it suffices to show that each buyer $(F_{S'}, H_{\bS'})$ and each sub-buyer $(F_{S''}, H_{\bS''})$
has been charged at most $\frac{\epsilon}{6}A(F_{S'}, H_{\bS'})$ dollars.
By the above charging scheme,
the terms in LHS that are charged to buyer $(F_{S'}, H_{\bS'})$
are consistent with $(F_{S'}, H_{\bS'})$.
Using the same argument as in the previous section,
we can show the spending of $(F_{S'}, H_{\bS'})$ as a buyer
is at most
$$\frac{\epsilon}{nm}\MM(F_{S'}, H_{\bS'}) \Prob[F_{S'},  H_{\bS'}].$$
The spending of $(F_{S''}, H_{\bS''})$ as a sub-buyer can be bounded as follows:
\begin{align*}
&\sum_{(F_{S}, H_{\bS})\consistent (F_{S'}, H_{\bS'})}\frac{\Prob[F_{S}, H_{\bS}]}
{Z(F_{S}, H_{\bS})} \sum_{(F_{S'}, H_{\bS'})\consistent (F_{S''}, H_{\bS''})}
 \frac{\Prob[F_{S'},  H_{\bS'}]}
{Z(F_{S'}, H_{\bS'})} \\
&\cdot \Prob[ F_{S''},  H_{\bS''}]\cdot 2(m+2)\MM(F_{S''}, H_{\bS''}) \\
=&\, 2(m+2)\MM(F_{S''}, H_{\bS''}) \Prob[F_{S''},  H_{\bS''}]
\cdot \sum_{(F_{S}, H_{\bS})\consistent (F_{S'}, H_{\bS'})}\frac{\Prob[F_{S}, H_{\bS}]}
{Z(F_{S}, H_{\bS})} \\
&\cdot \sum_{(F_{S'}, H_{\bS'})\consistent (F_{S''}, H_{\bS''})} \frac{\Prob[F_{S'},  H_{\bS'}]}
{Z(F_{S'}, H_{\bS'})}\\
\leq &\,2(m+2)\MM(F_{S''}, H_{\bS''}) \Prob[F_{S''},  H_{\bS''}]
\cdot \sum_{(F_{S}, H_{\bS})\consistent (F_{S'}, H_{\bS'})}
 \sum_{(F_{S'}, H_{\bS'})\consistent (F_{S''}, H_{\bS''})} \frac{\Prob[F_{S'},  H_{\bS'}]}
{Z(F_{S'}, H_{\bS'})} \\
\leq &\,2(m+2)\MM(F_{S''}, H_{\bS''}) \Prob[F_{S''},  H_{\bS''}]
\cdot m^2
 \sum_{(F_{S'}, H_{\bS'})\consistent (F_{S''}, H_{\bS''})} \frac{\Prob[F_{S'},  H_{\bS'}]}
{Z(F_{S'}, H_{\bS'})} \\
\leq &\, 2(m+2)\MM(F_{S''}, H_{\bS''}) \Prob[F_{S''},  H_{\bS''}]\cdot m^{2}
\sum_{v\in \bS''} \frac{\Prob[v\notin \Home(v)]}{\Prob[v\in \Home(v)]} \\
\leq &\, \frac{\e}{6}\MM(F_{S''}, H_{\bS''}) \Prob[F_{S''},  H_{\bS''}]
\end{align*}
%To see the second and the third inequality,
%for a fixed vertex $v$, consider the quantity
%$$
%\sum_{(F_{S'}, H_{\bar{S}'})\consistent (F_{S''}, H_{\bar{S}''}), S''=S'\setminus \{v\}}
%\frac{\Prob[F_{S'}, H_{\bar{S}'}]}{Z(F_{S'}, H_{\bar{S}'})}
%$$
%By the definition of $Z$, we can see that denominators of all terms are in fact the same.
%Then it is not hard to see the quantity is at most $\frac{\Prob[v\notin \Home(v)]}{\Prob[v\in \Home(v)]}$.
Note that for each $(F_{S'}, H_{\bar{S}'})$, there are at most $m^2$ different $(F_{S}, H_{\bar{S}})$ such that $(F_{S}, H_{\bar{S}})\consistent (F_{S'}, H_{\bar{S}'})$. So we have the second inequality.
The third inequality can be seen by canceling out same multiplicative terms from the numerators and the denominators, as
in Lemma~\ref{lm:mstcharge}.
\qed
\end{proof}


\section{Minimum Cycle Covers}
\label{sec:cc}
%We consider the locational uncertainty version of the minimum cycle cover, where the existence of each node is
%certain but its location is stochastic.
In this section, we consider the minimum length cycle cover problem.
In the deterministic version of the cycle cover problem,
we are asked to find a collection of vertex-disjoint cycles such that
every vertex is in one cycle and the total length is minimized.
Here we assume that every cycle contains at least two nodes.
If a cycle contains exactly two nodes, the length of the cycle is two times the
distance between these two nodes.
The problem can be solved in polynomial time by
reducing the problem to a minimum bipartite perfect matching problem.
\footnote{
If we require each cycle consist at least three nodes,
the problem is still poly-time solvable by a reduction to minimum perfect matching by Tutte~\cite{tutte54}.
Hartvigsen~\cite{harvigsen84} obtained a  polynomial time algorithm for
minimum cycle cover with each cycle having at least 4 nodes
Cornu\'{e}jols and Pulleyblank \cite{corn1980} have reported that Papadimitriou showed the NP-completeness of
minimum cycle cover with each cycle having at least 6 nodes.
}
W.l.o.g., we assume no two edges in $\P \times \P$ have the same length.
For ease of exposition, we assume that for each point, there is only one node that may realize
at this point.
In principle, if more than one nodes may realize at the same point, we can
create multiple copies of the point co-located at the same place,
and impose a distinct infinitesimal distance between every pair of copies,
to ensure no two edges have the same distance.

%Let $\p_{vs}=\Prob[v \realize s]$, i.e., the probability that node $v$ is present at point $s$.
%Since node $v$ is present with certainty, we have $\sum_{s\in P} \p_{vs}=1$.

\begin{theorem}
\label{thm:cc}
There is an FPRAS for estimating the expected length of
the minimum length cycle cover in both the locational uncertainty model
and the existential uncertainty model.
\end{theorem}

We need the notion of the nearest neighbor graph, denoted by $\NN$ .
For an undirected graph, an edge $e=(u,v)$ is in the nearest neighbor graph
if $u$ is the nearest neighbor of $v$, or vice versa.
We also use $\NN$ to denote its length.
$\Exp[\NN]$ can be computed exactly in polynomial time \cite{kamousi2011stochastic}.
\eat{
In fact, this can be seen by noting that
$
\Exp[\NN]=\sum_{e}c_e \cdot \Prob[e\in \NN]
$
and
$\Prob[e\in \NN] $ can be computed in poly-time.
To see this, note that $e=(s,t)$ is in $\NN$ if and only if at least one of the following two events happen
(1) both points $s$ and $t$ are chosen and no other points are chosen in $\B(s, \dist(e))$ and
(2) both points $s$ and $t$ are chosen and no other points are chosen in $\B(s, \dist(e))$.
}
As a warmup, we first show that $\Exp[\NN]$ is a 2-approximation of $\Exp[\CC]$ in the following lemma.
\begin{lemma}
\label{lmNNCC}
$
\Exp[\NN]\leq \Exp[\CC] \leq 2\Exp[\NN].
$
\end{lemma}

\begin{proof}
We show $\NN\leq \CC\leq 2\NN$ for each possible realization.
We prove the first inequality.
For each node $u$, there are two edges incident on $u$.
Suppose they are $e_{u1}$ and $e_{u2}$. We have
$
\CC=\frac{\sum_{u}(\dist(e_{u1})+\dist(e_{u2}))}{2}\geq \NN.
$
The second inequality can be seen by doubling all edges in $\NN$
and the triangle inequality. \qed
\end{proof}

We denote the longest edge in $\NN$ (and also its length) by  $\L$.
Note that $\L$ is also a random variable.
By the law of total expectation, we estimate $\Exp[\CC]$ based on the following formula:
$$
\Exp[\CC]=\sum_{e\in \P\times\P}\Prob[\L=e]\cdot \Exp[\CC\mid \L=e]
$$
It is obvious to see that $\frac{\NN}{n}\leq \L\leq \NN$.
Combined with Lemma~\ref{lmNNCC}, we have that
\begin{align}
\label{eq:CCbound}
\dist(e)\leq \Exp[\CC\mid \L=e]\leq 2n\dist(e).
\end{align}
However, it is not clear to us how to estimate $\Prob[\L=e]$
and how to take samples conditioning on event $\L=e$ efficiently.
To circumvent the difficulty, we consider some simpler events and condition $\L=e$
on those simpler events.
%Also note that there is less than $m^2$ distinct lengths of edges between points, so we only need to consider less than $m^2$ different length $l$.
%Here we assume no two edges have the same length, since if there are two edges have the same length, we can always make one of them increase
%very little such as $\frac{\epsilon \Exp[\NN]}{m^5}$ ($\Exp[\NN]$ is the lower bound of $\Exp[\CC]$) and it increases $\Exp[\CC]$ by at most a $\frac
%{\epsilon}{m}$ factor. \\
Consider a particular edge $e=(s,t) \in \P\times\P$.
Denote $N_s(t)$ as the event that the nearest neighbor of $s$ is $t$ and $N_t(s)$ as the event that the nearest neighbor of $t$ is $s$.
Let $L_{st}$ be the event the longest edge $\L$ in $\NN$ is $e(s,t)$.
Let $A_s(t)=N_s(t)\wedge L_{st}$. First we write
\begin{align*}
\Exp[\CC\mid \L=e]\cdot \Prob[\L=e] =& \Exp[\CC\mid A_s(t)\vee A_t(s)]\cdot\Prob[A_s(t)\vee A_t(s)] \\
= & \Exp[\CC\mid A_s(t)]\cdot \Prob[A_s(t)]+ \Exp[\CC\mid A_t(s)]\cdot \Prob[A_t(s)]\\
  &- \Exp[\CC\mid A_s(t)\wedge A_t(s)]\cdot \Prob[A_s(t)\wedge A_t(s)]
\end{align*}
Now, we show how to estimate $\Exp[\CC\mid A_s(t)]\cdot \Prob[A_s(t)]$ for each edge $e(s,t)$.
The other two terms can be estimated in the same way.
Also notice that the third term is less than the first and the second terms.
Therefore, for any points $s$ and $t$, we have the following fact which is useful later:
\begin{align}
\label{eq:CCbound2}
\Exp[\CC]\geq \Exp[\CC\mid \L=e]\cdot \Prob[\L=e]\geq \Exp[\CC\mid A_s(t)]\cdot \Prob[A_s(t)].
\end{align}
Moreover, we have that
\begin{align*}
\Exp[\CC\mid A_s(t)]\cdot\Prob[A_s(t)]=\Exp[\CC\mid A_s(t)]\cdot\Prob[L_{st}\wedge N_s(t)]
\\=\Exp[\CC\mid A_s(t)]\cdot \Prob[L_{st}\mid N_s(t)]\cdot \Prob[N_s(t)]
\end{align*}
Suppose $v$ is the only point that may realize to $s$
and $u$ is the only point that may realize to $t$.
We use $\B$ as a shorthand notation for $\B(s,\dist(s,t))$.
We first observe that $\Prob[N_s(t)]$ can be computed exactly in poly-time as follows:
$$
\Prob[N_s(t)]=p_{vs}\cdot p_{ut}\cdot \prod_{w\ne v,u} \bigl(1-p_w(\B) \bigr)
$$
Also note that we can take samples conditioning on the event $N_s(t)$
(the corresponding probability distribution for node $v$ is:
$\Prob[v\realize r \mid N_s(t)] = \frac{p_{vr}}{1-p_w(\B)}$).

\vspace{0.2cm}
\noindent
\topic{ Estimating $\Exp[\,\CC\mid A_s(t)\,]\cdot \Prob[L_{st}\mid N_s(t)]$}
Next, we show how to estimate $\Exp[\CC\mid A_s(t)]\cdot\Prob[L_{st}\mid N_s(t)]$.
The high level idea is the following.
We take samples conditioning on $N_s(t)$.
If $\Prob[L_{st}\mid N_s(t)]$ is large (i.e., at least $1/\poly(nm)$),
we can get enough samples satisfying $L_{st}$, thus $A_s(t)$.
Therefore, we can get $(1\pm\e)$-approximation for
both $\Prob[L_{st}\mid N_s(t)]$ and $\Exp[\CC\mid A_s(t)]$ in poly-time
(we also use the fact that if $A_s(t)$ is true, $\CC$ is at least $\dist(s,t)$ and at most $n\dist(s,t)$).
However, if $\Prob[L_{st}\mid N_s(t)]$ is small, it is not clear how to obtain a reasonable
estimate of this value.
In this case, we show the contribution of the term to our final answer is extremely small
and even an inaccurate estimation of the term will not affect our answer
in any significant way with high probability.

Now, we elaborate the details.
We iterate the following steps for $N$ times ($N=O(\frac{n^2m^3}{\e^3}(\ln n+\ln m))$ suffices).
\begin{itemize}
\item Suppose we are in the $i$th iteration.
We take a sample $G_i$ of the stochastic graph conditioning on the event $N_{s}(t)$.
We compute the nearest neighbor graph $\NN(G_i)$ and
the minimum length cycle cover $\CC(G_i)$ of $G_i$.
If $e(s,t)$ is the longest edge in $\NN(G_i)$, let $I_i=1$.
Otherwise $I_i=0$.
\end{itemize}
Our estimate of $\Exp[\,\CC\mid A_s(t)\,]\cdot \Prob[L_{st}\mid N_s(t)]$
is the following:
$$
\left( \frac{\sum_{i=1}^{N} I_i \cdot\CC(G_i) }{\sum_{i=1}^N I_i} \right)\left( \frac{\sum_{i=1}^N I_i}{N} \right)
=
\frac{\sum_{i=1}^{N} I_i\cdot \CC(G_i) }{N}
$$
It is easy to see the expectation of $\frac{\sum_{i=1}^{N} I_i\cdot \CC(G_i) }{N}$ is exactly
$\Exp[\,\CC\mid A_s(t)\,]\cdot \Prob[L_{st}\mid N_s(t)]$.

We distinguish the following two cases:
\begin{enumerate}
\item
$ \Prob[L_{st}\mid N_s(t)]\geq \frac{\epsilon}{2nm^3}$.
By Lemma~\ref{lm:chernoff}, $\frac{\sum_{i=1}^N I_i}{N}\in (1\pm \epsilon)\Prob[L_{st}\mid N_s(t)]$ with high probability.
%Moreover, we can get $\sum_{i=1}^{N} I_i \geq \Omega\Bigl(\frac{n}{\e^2}(\ln n+\ln m)\Bigr)$ with high probability.
In this case, we have enough successful samples (samples with $I_i=1$) to guarantee that
$\frac{\sum_{i=1}^{N} I_i \CC(G_i) }{\sum_{i=1}^N I_i}$
is a ($1\pm \e$)-approximation of $\Exp[\,\CC\mid A_s(t)\,]$ with high probability,
again by Lemma~\ref{lm:chernoff}.
We note that under condition $A_s(t)$, we have poly-bounded
since $\CC$ is at least $\dist(s,t)$ and at most $n\dist(s,t)$.
\item
$\Prob[L_{st}\mid N_s(t)]< \frac{\epsilon}{2nm^3}$.
%Then by Markov's inequality, $\Prob\left[\frac{\sum_{i=1}^N I_i}{N}\geq \frac{\e}{(nm)^{3}}\right]\leq \frac{1}{nm}$.
We note that $I_i=0$ means that while $N_s(t)$ happens, the longest edge $\L$ in $\NN$ is longer than $e(s,t)$.
Suppose $e(s',t')$ is the edge with the maximum $\Prob[L_{s't'}|N_s(t)]$.
Since $\Prob[L_{st}\mid N_s(t)]\leq \frac{\epsilon}{2nm^3}$, $e(s',t')$ must be different from $e(s,t)$
and $\Prob[L_{s't'}\mid N_s(t)]\geq \frac{2nm^2}{\e}\Prob[L_{st}\mid N_s(t)]$.
Hence, we have that
\begin{align*}
\Exp[\CC\mid A_s(t)]\cdot\Prob[A_s(t)]&=
\Exp[\CC\mid A_s(t)]\cdot \Prob[L_{st}\mid N_s(t)]\cdot \Prob[N_s(t)] \\
&\leq n \cdot \dist(s,t) \cdot \frac{\e}{2nm^2}\cdot \Prob[L_{s't'}\mid N_s(t)]\cdot \Prob[N_s(t)] \\
&\leq \frac{\e}{2m^2}\cdot \dist(s',t') \cdot \Prob[L_{s't'}\mid N_s(t)]\cdot \Prob[N_s(t)] \\
&\leq \frac{\e}{2m^2}\cdot \Exp[\,\CC\mid A_{s'}(t')] \cdot \Prob[L_{s't'}] \\
&\leq \frac{\e}{2m^2}\cdot \Exp[\CC]
\end{align*}
The first and third inequalities are due to \eqref{eq:CCbound} and the fourth are due to \eqref{eq:CCbound2}.
By Chernoff Bound, we have that
$$
\Prob\left[\frac{\sum_{i=1}^{N} I_i\cdot \CC(G_i) }{N}\geq \frac{\e}{m^2}\cdot \Exp[\CC]\right]\leq \frac{e^{-n}}{m^2}
$$
Then, with probability at least $1-\poly(\frac{1}{n})$,
the contribution from all such edges is less than $\e\Exp[\CC]$.
\end{enumerate}

Summing up, we have obtained Theorem~\ref{thm:cc}.


%\vspace{-0.2cm}
%\topic{Running time:}
%Overall, we need to take $O(n^2m^3\e^{-3}\ln(nm)$ samples.
%We need to compute the minimum cost cycle cover, which reduces to the problem of
%computing the minimum cost perfect matching in a general graph.

%\vspace{0.2cm}

Finally, we remark that our algorithm also works in presence of both locational uncertainty and node uncertainty, i.e.,
the existence of each node is a Bernoulli random variable.
It is not hard to extend our technique to handle the case where each cycle is required to contain at least three nodes.
This is done by considering the longest edge in the $2\NN$ graph (each vertex connects to the nearest and second nearest
neighbors).
%However, it is impossible to get a FPRAS if we require each cycle contain at least four nodes since
%computing the minimum length cycle cover under the same constraint is NP-hard.
%We defer the details to a later version of the paper.
The extension is fairly straightforward and we omit the details here.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\eat{
In fact, we can see that
$$
\Prob[N_s(t)]=\sum_{v\in \V} p_{vs} \Bigl( \prod_{u\ne v}  \pi_u \Bigr) \Bigl(1-\prod_{u\ne v} \frac{p_{ut}}{\pi_u}\Bigr)
$$
Now, we focus on how to estimate $\Exp[\CC\mid A_s(t)]\cdot \Prob[L_{st}]$.
We first observe that
$$
N_s(t)=\bigvee_{u\ne v} N_{u\realize s}(v\realize t).
$$
where $N_{u\realize s}(v\realize t)=N_s(t)\wedge u\realize s \wedge v\realize t$.
The idea is similar to the algorithm for estimating the size of the union of a collection of sets,
given that we know the cardinality of each set and can sample uniformly from each of them (see e.g., \cite[Ch. 10]{mitzenmacher2004probability}).
\vspace{0.2cm}
\noindent
{\bf Estimating $\Exp[\CC\mid A_s(t)]\cdot \Prob[L_{st}]$:}
We iterate the following steps for $N$ times.
\begin{enuemrate}
\item Suppose we are in the $i$th iteration.
We first sample an pair $(v,u)\in \V\times \V$ with probability
$$
%\frac{\Prob[N_{u\realize s}(v\realize t)]}
%{\sum_{u'\ne v'}\Prob[N_{u'\realize s}(v'\realize t)]}
\Prob[N_{v\realize s}(u\realize t)] \Big/
\sum_{v'\ne u'}\Prob[N_{v'\realize s}(u'\realize t)]
$$
Note that $\Prob[N_{v\realize s}(u\realize t)]=p_{vs}\cdot p_{ut}\cdot \prod_{w\ne v,u} \pi_w$.
\item
We take a sample $G$ of the stochastic graph conditioning on the event $N_{v\realize s}(u\realize t)$.
We compute the minimum length cycle cover of $G$.
If $e(s,t)$ is the longest edge in the cycle cover, let $N_0$
\end{enumerate}
}%\eat

%\vspace{-0.3cm}
\section{Convex Hull (2D)}
\label{sec:ch}

We demonstrate the problem of computing the expected aero of the convex hull (2D) under the {\em existential uncertainty model}. Given a set of points $\P=\{s_1, \ldots, s_m\}$ on a plane, where each point $s_i\in \P$ is present with probability $p_i$. For any nonnegative integer $i$ and a point set $H$, let $H\A{i}$ to denote the event that exactly $i$ points are present in $H$.

We use $\CH$ to denote the the expected area of the convex hull in the realized graph. Our \core\ recipe works well for this problem.
Firstly, we find the \core\ $\H=\{s_i\mid p_i\geq \frac{\e}{m^2}\}$. Let $\calF=\P\setminus \H$. Then we could rewrite $\Exp[\CH]$ by $\sum_{0\leq i\leq m}\Prob[\calF\A{i}]\cdot \Exp[\CH\mid \calF\A{i}]$. We need the following lemma first.

\begin{lemma}
\label{lm:4ch}
Given a convex hull with no less than 4 points whose aero is $A$. There exists 4 points on the convex hull, where the aero of the convex hull constructed by these 4 points is at least $A/2$.
\end{lemma}

\begin{proof}
We find the farthest pair ($s_1,s_2$) on the convex hull at first. Connect $s_1$ and $s_2$ to get a straight line $l$. On both sides of $l$, find a point each on the convex hull which is the farthest from $l$. Suppose these 2 points are $s_3$ and $s_4$, then by the property of convex hull, the aero of the convex hull constructed by $s_1,s_2,s_3,s_4$ is at least $A/2$.
\qed
\end{proof}

By Lemma~\ref{lm:4ch}, we could use the similar argument as $\Prob[\CP\leq 1]$ to show the contribution of the term $\sum_{5\leq i\leq n}\Prob[\calF\A{i}]\cdot \Exp[\CH\mid \calF\A{i}]$ are negligible compared to the fifth term. Briefly speaking, for $i\geq 5$ and a realized graph $C$ conditioning on $\calF\A{i}$, we could find out a realized graph conditioning on $\calF\A{i-1}$ which is of aero at least $\CH(C)/2$.
Then we just use the Monte Carlo method to estimate the first five terms and achieve an $\FA$ for the problem.

\section{Statistics under Gaussian distribution}
\label{sec:gaussian}
In this section, we consider a continuous version for estimating statistics such as closest pair, minimum spanning tree, minimum perfect matching and minimum cycle cover.
We use the term {\em nodes} to refer to the vertices $\V$ ($|\V|=n$). The location of each node $v_i\in \V$ independently follows its own multivariate Gaussian distribution $\calN(\mu_i,\sum_{i})$ (with mean $\mu_i\in \R^m$ and covariance matrix $\Sigma_{i}\in \mathbb{R}^{m\times m}$). Note that this setting is a continuous version of the {\em locational uncertainty model}. We consider the problem of estimating $\Exp[\CP]$ in this continuous version as an example.

At first, we represent each covariance matrix $\Sigma_{i}$ as a vector $\Psi_i=((e_{i,1},\sigma_{i,1}),\ldots,(e_{i,m},\sigma_{i,m}))$, where $e_{i,j}$ ($j\in [m]$) are a set of orthogonal basis vectors in $\R^m$, and $\sigma_{i,j}\in \R^+$ for all $j\in [m]$. It means that the location of node $v_i$ has mean $\mu_i$ and follows an independent Gaussian distribution on each direction $e_{i,j}$ ($j\in [m]$) with variance $\sigma_{i,j}$. Without loss of generality, we assume that $\sigma_{i,1}\geq \sigma_{i,2}\geq \ldots \geq \sigma_{i,m}$ for all $i\in [n]$. Note that $\sigma_{i,1}$ is bounded in $[\min_{j\in [m]}|\Sigma_{i,jj}|,\max_{j\in [m]}|\Sigma_{i,jj}|]$ where $\Sigma_{i,jj}$ is the $j$th number on the diagonal of $\Sigma_i$.

Given a polytope $H\subset \R^m$, we define $v\realize H$ the location of the node $v$ is in $H$. For each node $v_i$, we define a box $B_i=\{x\in \R^m \mid |\langle x-\mu_i,e_{i,j}\rangle |\leq (\sqrt{2\ln (\frac{mn^2}{\epsilon})}+3)\sigma_{i,j}, j\in [m]\}$. Then we focus on the following theorem.

\begin{theorem}
\label{thm:estCPgaussian}
There is an FPRAS for estimating the expected distance between
the closest pair of nodes while the location of each node independently follows its own multivariate Gaussian distribution.
\end{theorem}

To prove Theorem~\ref{thm:estCPgaussian}, we want to show that by taking enough samples, we have a good approximation for $\Exp[\CP]$. Thus, the main idea is to give $\Exp[\CP]$ a lower bound and show that the instance that $\CP$ is too large is negligible. We first give the following lemmas to give a lower bound for $\Exp[\CP]$.

\begin{lemma}
\label{lm:box}
For each node $v_i$, we have $\Prob[v_i\realize B_i]\geq 1-0.03\epsilon/n^2$.
\end{lemma}

\begin{proof}
For one dimensional Gaussian distribution $X\sim \calN(\mu,\sigma)$, we show that
$\Prob[|X-\mu|\leq (\sqrt{4\ln n}+3)\sigma] \geq 1-0.03/n^2$.
Note that
$$\Prob[X-\mu> 3\sigma] =\int_{\mu+3\sigma}^{+\infty}\frac{1}{\sigma\sqrt{2\pi}}\exp^{-\frac{(x-\mu)^2}{2\sigma^2}}dx\leq 0.015 $$
Then we have
\begin{align}
&\Prob[X-\mu>(\sqrt{4\ln t}+3)\sigma] = \int_{\mu+(\sqrt{4\ln t}+3)\sigma}^{+\infty}\frac{1}{\sigma\sqrt{2\pi}}\exp^{-\frac{(x-\mu)^2}{2\sigma^2}}dx \\
=& \int_{\mu+3\sigma}^{+\infty}\frac{1}{\sigma\sqrt{2\pi}}\exp^{-\frac{(x+\sqrt{4ln t}\sigma-\mu)^2}{2\sigma^2}}dx \leq \frac{1}{t^2}\int_{\mu+3\sigma}^{+\infty}\frac{1}{\sigma\sqrt{2\pi}}
\exp^{-\frac{(x-\mu)^2}{2\sigma^2}}dx\leq 0.015/t^2
\end{align}
So we have $\Prob[|X-\mu|\leq (\sqrt{4\ln n}+3)\sigma] \geq 1-0.03/n^2$. By the definition of box $B_i$, we have
$$\Prob[v_i\realize B_i]\geq (1-\frac{0.03\epsilon}{mn^2})^m \geq 1-0.03\epsilon/n^2$$
\qed
\end{proof}

\begin{lemma}
\label{lm:lbestCP}
$\Exp[\CP]\geq \frac{2}{3}\min\limits_{i,j\in[n]}\max\{\dist(\mu_i,\mu_j)-(\sqrt{2\ln (\frac{mn^2}{\epsilon})}+3)(\sigma_{i,1}+\sigma_{j,1}), \frac{\max\{\sigma_{i,1},\sigma_{j,1}\}}{4n^2}\}$.
\end{lemma}

\begin{proof}
On one hand, by Lemma~\ref{lm:box}, for any two nodes $v_i,v_j$ ($i,j\in [n]$), we have $\Prob[\dist_{i,j}\geq \{\dist(\mu_i,\mu_j)-(\sqrt{2\ln (\frac{mn^2}{\epsilon})}+3)(\sigma_{i,1}+\sigma_{j,1})\}]\geq 1-0.06\epsilon/n^2$.

On the other hand, for any two nodes $v_i,v_j$ ($i,j\in [n]$), we assume that $\sigma_{i,1}\leq \sigma_{j,1}$. We fix the location $s$ of $v_i$, then we have
\begin{align}
&\Prob[\dist(v_i,v_j)\geq \frac{\sigma_{j,1}}{4n^2}\}\mid v_i\realize s] \geq \Prob[\dist(v_i,v_j)\geq \frac{\sigma_{j,1}}{4n^2}\mid v_i\realize \mu_j]\\
= &1-\Prob[\dist(v_j,\mu_j)<\frac{\sigma_{j,1}}{4n^2}]\geq  1-\frac{1}{2n^2}\cdot \frac{1}{\sqrt{2\pi}}\geq 1-\frac{1}{4n^2}
\end{align}
Thus for any two nodes $v_i,v_j$ ($i,j\in [n]$), we have $\Prob[\dist(v_i,v_j)\geq\max\{\dist(\mu_i,\mu_j)-(\sqrt{2\ln (\frac{mn^2}{\epsilon})}+3)(\sigma_{i,1}+\sigma_{j,1}), \frac{\max\{\sigma_{i,1},\sigma_{j,1}\}}{4n^2}\}]\geq 1-\frac{1}{3n^2}$. It is immediately that
$\Prob[\CP\geq \min\limits_{i,j\in[n]}\max\{\dist(\mu_i,\mu_j)-(\sqrt{2\ln (\frac{mn^2}{\epsilon})}+3)(\sigma_{i,1}+\sigma_{j,1}), \frac{\max\{\sigma_{i,1},\sigma_{j,1}\}}{4n^2}\}]\geq 1-\frac{n^2}{3n^2}=\frac{2}{3}$. So we prove the lemma.
\qed
\end{proof}

On the other hand, we rewrite $\Exp[\CP]=\Prob[\CP\leq c]\Exp[\CP\mid \CP\leq c]+\Prob[\CP>c]\Exp[\CP\mid \CP>c]$ for any $c>0$. Then we show that there exists a $c>0$ such that $\Prob[\CP>c]\Exp[\CP\mid \CP>c]$ is negligible.

\begin{lemma}
\label{lm:ubestCP}
For $c=\min\limits_{i,j\in[n]}\{\dist(\mu_i,\mu_j)+\frac{4n^2m}{\epsilon}(\sigma_{i,1}+\sigma_{j,1})\}$, we have $\Prob[\CP>c]\Exp[\CP\mid \CP>c]\leq \frac{\epsilon}{nm}\Exp[\CP]$.
\end{lemma}

\begin{proof}
Without loss of generality, we assume that $v_1,v_2\in \V$ are two nodes such that $c=\dist(\mu_1,\mu_2)+(\sqrt{2\ln (\frac{mn}{\epsilon})}+3)(\sigma_{1,1}+\sigma_{2,1})$.
Note that we have
$\Prob[\CP>c]\Exp[\CP\mid \CP>c]
\leq \Prob[\dist(v_1,v_2)>c]\Exp[\dist(v_1,v_2)\mid \dist(v_1,v_2)>c]$. Also note that if the event $\CP>c$ happens, either $\dist(v_1,\mu_1)>\frac{4n^2m}{\epsilon}\sigma_{1,1}$ or $\dist(v_2,\mu_2)>\frac{4n^2m}{\epsilon}\sigma_{2,1}$ happens. Thus, we have

\begin{align}
&\Prob[\dist(v_1,v_2)>c]\Exp[\dist(v_1,v_2)\mid \dist(v_1,v_2)>c] \\
\leq &\Prob[\dist(v_1,\mu_1)>\frac{4n^2m}{\epsilon}\sigma_{1,1}]\cdot \Exp[\dist(v_1,v_2)\mid \dist(v_1,\mu_1)>\frac{4n^2m}{\epsilon}\sigma_{1,1}]\\
&+\Prob[\dist(v_2,\mu_2)>\frac{4n^2m}{\epsilon}\sigma_{2,1}]\cdot
\Exp[\dist(v_1,v_2)\mid \dist(v_2,\mu_2)>\frac{4n^2m}{\epsilon}\sigma_{2,1}]\\
\end{align}

Note that

\begin{align}
&\Exp[\dist(v_1,v_2)\mid \dist(v_1,\mu_1)>\frac{4n^2m}{\epsilon}\sigma_{1,1}] \\
\leq & \Exp[\dist(v_1,\mu_1)+\dist(\mu_1,\mu_2)+\dist(v_2,\mu_2)\mid \dist(v_1,\mu_1)>\frac{4n^2m}{\epsilon}\sigma_{1,1}]\\
\leq &\Exp[\dist(v_1,\mu_1)\mid \dist(v_1,\mu_1)>\frac{4n^2m}{\epsilon}\sigma_{1,1}]
+\dist(\mu_1,\mu_2)+\sigma_{2,1}\\
\leq &\frac{4n^2m}{\epsilon}\sigma_{i,1}+\sigma_{1,1}
+\dist(\mu_1,\mu_2)+\sigma_{2,1}
\end{align}

By the same argument, we have
$$\Exp[\dist(v_1,v_2)\mid \dist(v_2,\mu_2)>\frac{4n^2m}{\epsilon}\sigma_{2,1}]
\leq  \frac{4n^2m}{\epsilon}\sigma_{2,1}+\sigma(2,1)
+\dist(\mu_1,\mu_2)+\sigma(1,1)$$

Also note that we have
$$\Prob[\dist(v_1,\mu_1)>\frac{4n^2m}{\epsilon}\sigma_{i,1}]+
\Prob[\dist(v_2,\mu_2)>\frac{4n^2m}{\epsilon}\sigma_{i,2}]\leq 2\exp^{-\frac{16n^4m}{\epsilon^2}}$$

Combine the inequalities, we conclude that $\Prob[\CP>c]\Exp[\CP\mid \CP>c]\leq 4c\cdot\exp^{-\frac{16n^4m}{\epsilon^2}} $. By Lemma~\ref{lm:lbestCP}, we have $$\frac{2}{3}\max\{\dist(\mu_i,\mu_j)-(\sqrt{2\ln (\frac{mn^2}{\epsilon})}+3)(\sigma_{1,1}+\sigma_{2,1}), \frac{\max\{\sigma_{1,1},\sigma_{2,1}\}}{4n^2}\}\leq \Exp[\CP]$$
It is not hard to show that $c\leq \frac{16n^6m^2}{\epsilon^2}\Exp[\CP]$, which completes the proof.
\qed
\end{proof}

Combine Lemma~\ref{lm:lbestCP} and \ref{lm:ubestCP}, we are ready to prove Theorem~\ref{thm:estCPgaussian} by Monte Carlo Method.

\begin{proof} (Theorem~\ref{thm:estCPgaussian}) We simply take $O(\frac{n^6m^2}{\epsilon^4}\ln(1/\delta))$ samples. We ignore all samples $G_i$ with $\CP(G_i)>c$. Then we compute the average length of the closest pair among these samples. By Monte Carlo Method, it is easy to show that we can obtain a $(1+\epsilon)$-approximation for $\Exp[\CP]$ with probability at least $1-\delta$.
\qed
\end{proof}

By the assumption that the location of each node independently follows its own multivariate Gaussian distribution, we can similarly give good approximations for $\Exp[\diam]$, $\Exp[\MST]$, $\Exp[\MM]$ and $\Exp[\CC]$. We only give an intuition here. For $\Exp[\diam]$ and $\Exp[\MST]$, the most important factor is the distance between the farthest pair. For $\Exp[\MM]$ and $\Exp[\CC]$, the most important factor is the distance between the closest pair. Then we can have a similar conclusion as Lemma~\ref{lm:lbestCP} and \ref{lm:ubestCP}, and show that taking enough samples can give a good approximation.






